Analytic and Gevrey class regularity for parametric semilinear reaction-diffusion problems and applications in uncertainty quantification

We investigate a class of parametric elliptic semilinear partial differential equations of second order with homogeneous essential boundary conditions, where the coefficients and the right-hand side (and hence the solution) may depend on a parameter. This model can be seen as a reaction-diffusion problem with a polynomial nonlinearity in the reaction term. The efficiency of various numerical approximations across the entire parameter space is closely related to the regularity of the solution with respect to the parameter. We show that if the coefficients and the right-hand side are analytic or Gevrey class regular with respect to the parameter, the same type of parametric regularity is valid for the solution. The key ingredient of the proof is the combination of the alternative-to-factorial technique from our previous work [1] with a novel argument for the treatment of the power-type nonlinearity in the reaction term. As an application of this abstract result, we obtain rigorous convergence estimates for numerical integration of semilinear reaction-diffusion problems with random coefficients using Gaussian and Quasi-Monte Carlo quadrature. Our theoretical findings are confirmed in numerical experiments.

==> Gauss_Legendre_experiment.tex <==
According to Theorem \ref{gevrey regularity for semilinear}, under appropriate assumptions the solution of the semilinear problem \eqref{variational form} inherits the Gevrey-$\delta$ class regularity from the coefficients and the right-hand side of this equation. To demonstrate this result in a numerical experiment, we first consider a simple model problem with a single scalar parameter $y$ being a random variable uniformly distributed in $[-1,1]$. The quantity of interest is defined as the integral 
 \begin{equation}\label{Elambda}
 	I(\cG) :=  \int_{-1}^1 \newpart{\cG}(y) \, dy,
 \end{equation}
where the functional $\newpart{\cG}(y) := \int_D u(\vx, y) \, d\vx$ is the average value of the solution $u$ in the computational domain $D= (0,1)^2$. Specifically, we consider the cubic nonlinearity $m=3$, \secondcmt{the forcing term $f= 3(\cos(2 \pi x_1)+1)(\cos(3\pi x_2)+1)$}, the unit diffusion coefficient $a\equiv 1$ and the reaction coefficient $b$ being either
\begin{equation}\label{def-b1}
	b^{(1)} (\vx,y) = 50(\cos^2(15\pi x_1+y^{10})+1)(\cos^2(17\pi x_2+y^{25})+1),
\end{equation}
or
\begin{equation}\label{def-b2}
	b^{(2)} (\vx,y) = \brac{\exp\brac{-\frac{x_1^2+x_2^2}{y+1}}+1}
	(\cos^2(15\pi x_1)+1)(\cos^2(17\pi x_2)+1).
\end{equation}
Since $m$ is odd and both $b^{(1)}$ and $b^{(2)}$ are nonnegative, Assumption \ref{Possitive b Assump} is valid and therefore corresponding solutions $u^{(1)}$ and $u^{(2)}$ of \eqref{variational form} are uniquely determined in $H^1_0(D)$ for every~$y\in [-1,1]$. Recall that $H^1_0(D)$ is continuously embedded in $L^1(D)$ and therefore, by Theorem \ref{gevrey regularity for semilinear}
\begin{equation}
|\partial^{\vnu}\cG| \leq \|\partial^{\vnu} u \|_{L^1(D)}
\leq C_0 \|\partial^{\vnu} u \|_{H^1_0(D)}
\leq C_0C_m^{-1}C_u \frac{(|\vnu|!)^\delta}{(\vR/\rho)^{\vnu}},
\end{equation}
i.e. $\newpart{\cG}=\newpart{\cG}^{(k)}$ is Gevrey-$\delta$ regular, where $\delta=\delta^{(k)}$ is determined by $b^{(k)}$, $k = 1,2$. \firstcmt{More precisely, we have}
\begin{align*}
\firstcmt{ b^{(1)}}&\firstcmt{ \in G^1([-1,1],L^{\infty}(D)),\quad
\cG^{(1)}\in G^1([-1,1],L^1(D)),\,}
\\
\firstcmt{  b^{(2)}}&\firstcmt{ \in G^2([-1,1],L^{\infty}(D)),\quad
\cG^{(2)}\in G^2([-1,1],L^1(D)).}
\end{align*}
%
%\tl{From the above setting, the solution $u$ would belong to $L^{\infty}(D)$, see e.g. \cite[Theorem 3.1]{AlejandroFranciscoEnriqueDaniel2021} and \cite[Theorem 4.8]{Trltzsch2010}}. 
We denote by $\{\xi_j,w_i\}_{j=1}^n$ the Gauss-Legendre quadrature points and weights and hereby the quadrature approximation to the quantity of interest~\eqref{Elambda}
 \begin{equation}
 	Q_n[\cG] :=  \sum_{j=1}^n w_j \newpart{\cG}(\xi_i).
 \end{equation}
According to \cite[Theorem 5.2]{ChernovSchwab2012} the asymptotic quadrature error is determined by the Gevrey class parameter of the data, that is $\delta^{(1)} = 1$ for \eqref{def-b1} and $\delta^{(2)} = 2$ for \eqref{def-b2}: $\exists C,r > 0$ independent on $n$ such that
 \begin{equation}\label{eps2}
 	\varepsilon_n^{(k)} := |I(\cG^{(k)}) - Q_n[\cG^{(k)}]| 
 	\leq 
 	C \exp( - r n^{1/\delta^{(k)}}), \qquad k=1,2.
 \end{equation}
Observe in particular that unlike $b^{(1)}$, the coefficient $b^{(2)}$ is not analytic near $y=-1$, see e.g. \cite[Section 5.2]{ChernovSchwab2012}), and this can be immediately detected by the reduced asymptotic convergence rate for the case~$k=2$. 


At every quadrature point $y = \xi_i$, we solve the variational problem \eqref{variational form} with the finite element method on a uniform triangular mesh with the mesh size $h=\sqrt{2}/128$. Since \eqref{variational form} is a nonlinear problem, we use the fixed-point iteration method \eqref{contracting mapping} with an absolute error tolerance of $10^{-14}$ with respect to the $H^1_0(D)$-seminorm. Since $I(\cG(u))$ is not available in closed form, we replace it by very fine quadrature approximations: $I^*(\cG(u^{(1)}))=Q_{50}[\cG(u^{(1)})]$ and $I^*(\cG(u^{(2)}))=Q_{150}[\cG(u^{(2)})]$ based on $n=50$ and $n=150$ Gauss-\secondcmt{Legendre} points respectively.

% As we can observe in the Figure 1, \tl{because of reaching machine precision ($2.2204 \cdot 10^{-16}$), quadrature error is stable when number of points is sufficiently large. }
 
\begin{figure}[h]
	\centerline{\includegraphics[width=\textwidth]{GL_int_u}}
	\caption{Quadrature error $\varepsilon^{(1)}_n$ (left) with respect to the number $n$ of quadrature points and Quadrature error $\varepsilon^{(2)}_n$ (right) with respect to $N = n^{1/2}$.}
	\label{fig1}
\end{figure}


In the left panel of Figure \ref{fig1}, the data points represent the quadrature error  $\varepsilon_n^{(1)}$ with respect to number of quadrature points $n$ and the reference line (dashed line)  shows the linear trend in semi-logarithmic scale. This agrees with \eqref{eps2} and $\delta^{(1)}=1$.
Similarly, the data points in the right panel of Figure 1 represent the quadrature error $\varepsilon_n^{(2)}$ with respect to the square root of the number of quadrature points $N :=n^{1/ \delta^{(2)}} = n^{1/2}$ in the semi-logarithmic scale. The reference line (dashed line) also shows the linear trend in semi-logarithmic scale. Clearly, this confirms \eqref{eps2} with $\delta^{(2)}=2$ and thereby demonstrates the meaning and validity of Theorem \ref{gevrey regularity for semilinear}.


==> Gevrey_regularity.tex <==
 The following definition of Gevrey-$\delta$ functions with countably many parameters will be used in our regularity analysis in Section \ref{sec: main result}.

\begin{definition} \label{def:G-delta-def}
	Let $\delta \geq 1$, $B$ be a Banach space, $I \subset \mR^\mN$ be an open domain and a function $f:I \to B$ be such that its $\vy$-derivatives $\partial^{\vnu} f:I \to B$ are continuous for all $\vnu \in \cF$. We say \firstcmt{the} function $f$ is of class Gevrey-$\delta$ if for each $y_0 \in I$ there exist an open set $J\subseteq I$, and strictly positive constants $\vR = (R_1,R_2,\dots) \subset \mR_{>0}^{\mN}$ and $C \in \mR_{>0}$ that the derivatives of $f$ satisfy the bounds
	\begin{equation}\label{G-delta-def}
		\|\partial^{\vnu} f(\vy)\|_B \leq \frac{C}{\vR^{\vnu}} (|\vnu|!)^\delta, \qquad \forall \vy \in J, \quad \forall \vnu \in \cF.
	\end{equation}
	In this case we write $f \in G^\delta(U,B)$.
\end{definition}

Definition \ref{def:G-delta-def} is also suitable for the case of finitely many parameters $\vy$. In particular, when $\vy = (y_1,\dots,y_M)$, $B = \mR$ or $\mC$ and $\delta=1$, the bound \eqref{G-delta-def} guarantees convergence of the power series of $f$ and therefore characterizes the class of analytic functions of $M$ variables, see e.g. \cite[Section 2.2]{Krantz2002} and \cite[Remark 2.6]{ChernovLe2023}. This property follows from the bound $|\vnu|! \leq M^{|\vnu|} \vnu!$ that is valid for a \secondcmt{multi-index} $\vnu$ with $M$ nonzero components.
Notice that otherwise estimate \eqref{G-delta-def} does not guarantee convergence of the power series of $f$. Moreover, the scale $G^\delta$ grows \firstcmt{monotonically} with $\delta$ in the sense of \eqref{Gdelta-nested}.
 
We now make an assumption on the coefficients, which, in particular, ensure that the solution of the semilinear problem \eqref{gen equation} is Gevrey-class regular.
	\begin{assumption} \label{Assumption}
		For all fixed values $\vy\in U \firstcmt{\subset} \mR^s$ with $s<\infty$, the coefficients $a(\vy),b(\vy) \in L^\infty(D)$ and $f(y)\in V^*$. The functions \firstcmt{$a$, $b$} are of Gevrey class $G^\delta(U,L^{\infty}(D))$ and \firstcmt{$f$} is of Gevrey class $G^\delta(U,V^*)$, i.e. for all $\vnu\in \mN^s$ there exist $\vR$ independent of $s$ such that
		\begin{align*}
			\norm{\partial^{\vnu} a(\vy)}{L^\infty(D)}
			\leq
			\frac{\overline{a}}{2}
			\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}} , \qquad
			\norm{\partial^{\vnu} b(\vy)}{L^\infty(D)}
			\leq
			\frac{\overline{b}}{2}
			\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}} , \qquad
			\norm{\partial^{\vnu} f(\vy)}{V^*}
			\leq
			\frac{\overline{f}}{2}
			\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}}  .
		\end{align*} 
	\end{assumption}
	Notice that for $\vnu = \vzero$ Assumption \ref{Assumption} agrees with the upper bounds in \eqref{ab-bounds}. Notice also that the components of $\vR$ are readily scaled by the factor of $2$. This leads to no loss of generality, but helps to shorten the forthcoming expressions. 
	For example, in view of \eqref{ff-estimates} Assumption \ref{Assumption} immediately implies
\begin{align}\label{abf assumption}
	\norm{\partial^{\vnu} a(\vy)}{L^\infty(D)}
	\leq
	\frac{\overline{a} \gdnota{\abs{\vnu}}}{\vR^{\vnu}} (\abs{\vnu}!)^{\delta-1} , \qquad
	\norm{\partial^{\vnu} b(\vy)}{L^\infty(D)}
	\leq
	\frac{\overline{b} \gdnota{\abs{\vnu}}}{\vR^{\vnu}}
	(\abs{\vnu}!)^{\delta-1} , \qquad
	\norm{\partial^{\vnu} f(\vy)}{V^*}
	\leq
	\frac{\overline{f} \gdnota{\abs{\vnu}}}{\vR^{\vnu}}(\abs{\vnu}!)^{\delta-1} .
\end{align}

The definition of the norms used above is standard \secondcmt{and} will be recalled in the beginning of the next section.


==> Numerical_experiment.tex <==
Let the domain $D= (0,1)^2$ and consider the problem \eqref{gen equation} with $a\equiv 1$, $f= 3(\cos(2 \pi x_1)+1)(\cos(3\pi x_2)+1)$, $m=3$ and $b$ is one of following functions 
\begin{equation}\label{def-b1}
b^{(1)} (\vx,y) = 50(\cos^2(15\pi x_1+y^{10})+1)(\cos^2(17\pi x_2+y^{25})+1),
\end{equation}
\begin{equation}\label{def-b2}
b^{(2)} (\vx,y) = \brac{\exp\brac{-\frac{x_1^2+x_2^2}{y+1}}+1}
(\cos^2(15\pi x_1)+1)(\cos^2(17\pi x_2)+1).
\end{equation}
Here $y$ is a scalar real parameter with the range $[-1,1]$. Since $m$ is odd and both $b^{(1)}$ and $b^{(2)}$ are nonnegative, Assumption \ref{Possitive b Assump} is valid and therefore corresponding solutions $u^{(1)}$ and $u^{(2)}$ of \eqref{variational form} are uniquely determined in $V$ for every $y\in [-1,1]$. Consider the functional $\cG(u)(y) := u(\vx_0,y)$, ${\vx}_0=(0.5,0.5)$, i.e. the point evaluation in the center of the computational domain $D$. Our goal is to compute numerically the (rescaled) expectation of $\cG(u)(y)$ if $y$ is a scalar real random variable uniformly distributed in $[-1,1]$
\begin{equation}\label{Elambda}
I(\cG(u)) :=  \int_{-1}^1 u(x_0,y) \, dy.
\end{equation}
Since the solution $u$ is not available in closed form, the integral \eqref{Elambda} can be approximated by numerical quadrature, e.g. the Gauss-Legendre quadrature, which is a reasonable choice for the case of a single real-valued parameter $y$. Let $\{\xi_i,w_i\}_{i=1}^n$ be the nodes and weights of the $n$-point Gauss-Legendre quadrature
\begin{equation}
Q_n[\cG(u)] :=  \sum_{i=1}^n w_i u(\vx_0,\xi_i).
\end{equation}
We are interested in the behaviour of the quadrature error
\begin{equation}
\varepsilon_n = |I(\cG(u)) - Q_n[\cG(u)]|
\end{equation}
with increasing $n$. It is known that the convergence of $\varepsilon_n$ is strongly related to the regularity of $u$ with respect to $y$. In particular \cite[Theorem 5.2]{ChernovSchwab2012} implies that
\begin{equation}
\varepsilon_n \leq C \exp( - r n^{1/\delta}).
\end{equation}
with positive constants $C$ and $r$ independent of $n$ if $u$ is of class Gevrey-$\delta$.
\begin{itemize}
\item[(1)]
In the case of the analytic diffusion coefficient $b^{(1)}$ as in \eqref{def-b1} Theorem \ref{gevrey regularity for semilinear} implies that $u$ is analytic in $y$, i.e. $\delta = 1$, and therefore we expect
\begin{equation}\label{eps1}
\varepsilon_n^{(1)} \leq C \exp (-rn).
\end{equation}
\item[(2)] The diffusion coefficient $b^{(2)}$ is not analytic near $y = -1$, but is Gevrey-$\delta$ uniformly for all $y \in [-1,1]$ with $\delta \geq 2$, see \cite{ChenRodino1996} and \cite[Section 6]{ChernovSchwab2012}. Theorem \ref{gevrey regularity for semilinear} implies that $u$ is Gevrey-$\delta$ with the same $\delta = 2$ and hence we expect
\begin{equation}\label{eps2}
\varepsilon_n^{(2)} \leq C \exp (-rn^{1/2}).
\end{equation}
\end{itemize}
\begin{figure}[h]
	\centerline{\includegraphics[width=1\textwidth]{GL_fig}}
	\caption{Quadrature error $\varepsilon^{(1)}_n$ (left) with respect to the number $n$ of quadrature points and Quadrature error $\varepsilon^{(2)}_n$ (right) with respect to $N = n^{1/2}$.}
\end{figure}
In order to observe the behaviour predicted in \eqref{eps1} and \eqref{eps2} we solve deterministic equations \eqref{variational form} in every quadrature point $y = \xi_i$ on a very fine finite element grid having $16.129$ degrees of freedom. Since $I(\cG(u))$ is not available in closed form, we approximate it by a very fine Gauss-Legendre quadrature $Q_{n^*}[\cG(u)]$ with $n^* = 50$ quadrature nodes for $b^{(1)}$ and $n^* = 150$ quadrature nodes for $b^{(2)}$. As a solver for the nonlinear problem \eqref{variational form} we use the fixed-point iteration method \eqref{contracting mapping} with an absolute error tolerance of $10^{-14}$ with respect to the $H^1_0(D)$-seminorm.



In Figure 1, we plot the relative error $\varepsilon_n^{(1)}$ against the number of quadrature points $n$ in the semi-logarithmic scale. The reference line clearly shows the linear trend of the type $-r n + \log C$ and thereby confirms \eqref{eps1}.
 
In Figure 2, we plot the relative error $\varepsilon_n^{(2)}$ with respect to the square root of the number of quadrature points $N := n^{1/2}$ in the semi-logarithmic scale. Here we can also observe the linear trend of the type $-r N + \log C$. This confirms \eqref{eps2} and thereby demonstrates the meaning and validity of Theorem \ref{gevrey regularity for semilinear}.



%\begin{figure}[tb]
%\blankbox{.6\columnwidth}{5pc}
%\caption{This is an example of a figure caption with text.}
%\label{firstfig}
%\end{figure}


%\begin{figure}[h]
%	\centerline{\includegraphics[width=0.5\textwidth]{ex2_new-crop}}
%	\caption{{, where $n$ is the number of quadrature points.}}
%\end{figure}


==> Parametric_regularity_H2.tex <==
\subsection{Parametric regularity in $H^2(D)$ and pointwise estimates}

If $D$ is a convex Lipschitz domain and the coefficients $a,b$ and the right-hand side $f$ are sufficiently regular, it is actually possible to prove that estimates of the type \eqref{u H1 norm ref} remain valid in $H^2(D)$, and therefore in every space containing $H^2(D)$ with continuous embedding. In particular, pointwise estimates follow from $L^\infty(D)$ bounds. 

If the data are sufficiently regular (see Assumption \ref{Assumption1} below for the precise regularity assumptions), formal  
integration by parts in the variational formulation \eqref{variational form} delivers
\begin{equation*}
	\tl{C_m^2} \int_D a (\Delta u) v = \int_D (b u^m - \tl{C_m^2}\nabla a \cdot \nabla u - \tl{C_m} \,f) v.
\end{equation*}
The Leibniz product rule implies
\begin{equation*}
	\tl{C_m^2}\int_D a (\Delta \partial^{\vnu} u) v = \int_D \partial^{\vnu}(b u^m - \tl{C_m^2}\nabla a \cdot \nabla u - C_m f) v -
	\tl{C_m^2}\sum_{\vzero \leq \veta < \vnu }
	\binom{\vnu}{\veta} \partial^{\vnu-\veta} a (\Delta \partial^{\veta} u) v.
\end{equation*}
\tl{
We introduce the semi-norm as following
\begin{align}
	\abs{g}_{Z}= C_m \norm{\Delta g}{L^2(D)}.
\end{align}}
We now let $v = \Delta \partial^{\vnu} u$ and apply the triangle and the Cauchy-Schwarz inequalities. Recall that $a\geq 1$, and hence
\tl{
\begin{equation}\label{vnu-Delta-u}
	| \partial^{\vnu} u|_{Z}
	\leq \|\partial^{\vnu} (C_m^{-1} b u^m - C_m\nabla a \cdot \nabla u -  f)\|_{L^2(D)} 
	+ \sum_{\vzero \leq \veta < \vnu }
	\binom{\vnu}{\veta} \|\partial^{\vnu-\veta} a\|_{L^\infty(D)} | \partial^{\veta} u|_{Z}.
\end{equation}}

The second term admits Gevrey-$\delta$ bounds if $L^\infty(D)$ and $V^*$-norms for $a$ and $f$ in Assumption \ref{Assumption} are replaced by the $W^{1,\infty}(D)$ and $L^2(D)$-norms respectively. More precisely, we replace Assumption \ref{Assumption} by the following.
\begin{assumption} \label{Assumption1}
	For all fixed values $\vy\in U \in \mR^s$ with $s<\infty$, the coefficients $a(\vy) \in W^{1,\infty}(D)$, $b(\vy) \in L^\infty(D)$ and $f(y)\in L^2(D)$. Moreover, for all $\vnu\in \mN^s$ there exist positive constants $\vR=(R_1,R_2,\dots)$ independent of $s$ such that
	\begin{align*}
		\norm{\partial^{\vnu} a(\vy)}{W^{1,\infty}(D)}
		\leq
		\frac{\overline{a}}{2}
		\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}} , \qquad
		\norm{\partial^{\vnu} b(\vy)}{L^\infty(D)}
		\leq
		\frac{\overline{b}}{2}
		\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}} , \qquad
		\norm{\partial^{\vnu} f(\vy)}{L^2(D)}
		\leq
		\frac{\overline{f}}{2}
		\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}}  .
	\end{align*} 
	Assume moreover, that $m \in \mN$ is such that $H^1(D)$ is continuously embedded into $L^{2m}(D)$, i.e. $(d,2m-1) \in \cM$, see \eqref{cond: m d restriction}.
\end{assumption}
According to \eqref{ff-estimates} Assumption \ref{Assumption1} implies
\begin{align}\label{abf1 assumption}
	\norm{\partial^{\vnu} a(\vy)}{W^{1,\infty}(D)}
	\leq
	\frac{\overline{a} \gdnota{\abs{\vnu}}}{\vR^{\vnu}} (\abs{\vnu}!)^{\delta-1} , \qquad
	\norm{\partial^{\vnu} b(\vy)}{L^\infty(D)}
	\leq
	\frac{\overline{b} \gdnota{\abs{\vnu}}}{\vR^{\vnu}}
	(\abs{\vnu}!)^{\delta-1} , \qquad
	\norm{\partial^{\vnu} f(\vy)}{L^2(D)}
	\leq
	\frac{\overline{f} \gdnota{\abs{\vnu}}}{\vR^{\vnu}}(\abs{\vnu}!)^{\delta-1}.
\end{align}
The regularity of $\Delta \partial^{\vnu} u$ can now be established by bounding the terms in the right-hand side of \eqref{vnu-Delta-u}. The Leibniz general product rule and the triangle inequality yield for the first term 
\begin{equation*}
	\begin{split}
		\|\partial^{\vnu} (\tl{C_m^{-1}} b u^m - \tl{C_m} \nabla a \cdot \nabla u - f)\|_{L^2(D)}
		&\leq 
		 \|\partial^{\vnu} f\|_{L^2(D)}
		+
		\sum_{\vzero \leq \veta \leq \vnu} \binom{\vnu}{\veta}
		\big(
		\tl{C_m^{-1}}\|\partial^{\vnu-\veta} b\|_{L^\infty(D)} \|\partial^{\veta} (u^m)\|_{L^2(D)}
		+ \|\nabla \partial^{\vnu-\veta} a\|_{L^\infty(D)} \| \partial^{\veta} u\|_{V}
		\big)\\
		&\leq 
		\|\partial^{\vnu} f\|_{L^2(D)}
		+
		\frac{(|\vnu|!)^{\delta-1}}{\vR^{\vnu}}
		\sum_{\vzero \leq \veta \leq \vnu} \binom{\vnu}{\veta}
		\big(
		4^{m-1}(C_{2m-1} C_m^{-1}  C_u)^m \tl{C_m^{-1}} \overline{b} +   C_u \overline{a}
		\big) \rho^{|\veta|} \gdnota{|\vnu-\veta|} \gdnota{|\veta|}\\
		&\leq 
		\tl{\big(
			4^{m}(C_{2m-1} C_u)^m C_m^{-m-1}  \overline{b}  + 4 C_u \overline{a} + \overline{f}
			\big)}
		\frac{  \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1},
	\end{split}
\end{equation*}
In the above estimate we used \eqref{multiindex-est-3} and the bounds
\begin{equation*}
	\|\partial^{\veta} u\|_{L^{2m}(D)} 
	\leq C_{2m-1}
	\|\partial^{\veta} u\|_{H^1_0(D)} 
	= C_{2m-1} C_m^{-1}
	\|\partial^{\veta} u\|_V
	\leq C_{2m-1} C_m^{-1}  C_u 
	\frac{ \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1},
\end{equation*}
i.e. the Sobolev embedding for $(d,2m-1) \in \cM$ and Theorem \ref{gevrey regularity for semilinear}. By Lemma \ref{upper bound for f derivative} this implies
\begin{equation*}
	\|\partial^{\veta} (u^m)\|_{L^2(D)} 
	=
	\|\partial^{\veta} (u^m)\|_{\LL{2m}{m}} 
	\leq 
	4^{m-1} (C_{2m-1} C_m^{-1}  C_u)^m
	\frac{ \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1}.
\end{equation*}
The argument can now be completed by an inductive argument, which is the subject of the following Theorem.

\begin{theorem}\label{thm:2}
	Suppose the assumptions of Theorem \ref{gevrey regularity for semilinear} hold and additionally Assumption \ref{Assumption1} is satisfied. Then $\Delta \partial^{\vnu} u \in L^2(D)$  for all $\vnu \in \cF$ and there holds
	\begin{equation}\label{Delta-u-derivative}
		| \partial^{\vnu}u|_{Z} \leq 
		\frac{2C_{\Delta} \tilde{\rho}^{|\vnu|} \gdnota{|\vnu|}}{\vR	^{\vnu}} (|\vnu|!)^{\delta-1},
	\end{equation}
	where $C_\Delta :=  \tl{
			4^{m}(C_{2m-1} C_u)^m C_m^{-m-1}  \overline{b}  + 4 C_u \overline{a} + \overline{f}
	}$ and $\tilde \rho := \max(6\overline{a},\rho)$.
\end{theorem}

\begin{proof}
	We prove the statement by induction. For $\vnu = \vzero$ we have by \eqref{vnu-Delta-u}
	\begin{equation*}
		\begin{split}
			| u|_{Z} &\leq \|\tl{C_m^{-1}} bu^m - \tl{C_m} \nabla a \cdot \nabla u -  f\|_{L^2(D)}
			\leq \tl{C_m^{-1}} \|b\|_{L^\infty(D)} \|u^m\|_{L^2(D)} 
			+ \|\nabla a\|_{L^2(D)} \|u\|_{V}
			+ \|f\|_{L^2(D)}\\
			&\leq 
			\tl{C_m^{-1}}\overline{b} \|u\|^m_{L^{2m}(D)}
			+\overline{a} \| u\|_{V} + \overline{f}
			\leq \tl{C_m^{-1}} \overline{b} (C_{2m-1}  C_m^{-1}\|u\|_V)^m
			+\overline{a} \|u\|_V + \overline{f} \\
			&\leq 
			\tl{C_m^{-1}}(C_{2m-1} C_m^{-1} C_u)^m \overline{b} 
			+ C_u \overline{a}  + \overline{f} \leq \tl{2 C_\Delta}
		\end{split}
	\end{equation*}
	
	The aim is now to prove \eqref{Delta-u-derivative}, assuming that it is valid for all derivatives of order strictly less than $\vnu$. From \eqref{vnu-Delta-u} and the bound below it, we readily have for $|\vnu|\geq 1$
	\begin{equation*}
		\begin{split}
			| \partial^{\vnu} u|_{Z}
			&\leq 
			C_\Delta
			\frac{  \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1} +
			\sum_{\vzero \leq \veta < \vnu }
			\binom{\vnu}{\veta} \|\partial^{\vnu-\veta} a\|_{L^\infty(D)} | \partial^{\veta} u|_{Z}\\
			&\leq 
			C_\Delta
			\frac{  \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1} +
			\sum_{\vzero \leq \veta < \vnu }
			\binom{\vnu}{\veta} 
			\frac{\overline{a}\gdnota{|\vnu-\veta|}}{\vR^{\vnu-\veta}} (|\vnu-\veta|!)^{\delta-1} 
			\frac{2C_\Delta \tilde{\rho}^{|\veta|}\gdnota{|\veta|}}{\vR^{\veta}} (|\veta|!)^{\delta-1} \\
			&\leq 
			2C_\Delta
			\frac{  \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1} \big(\frac{1}{2} + \frac{3\overline{a}}{\tilde \rho}\big).
		\end{split}
	\end{equation*}
	According to the definition of $\tilde \rho$ the term in the  parentheses is bounded by 1 and the claim of the theorem follows.
\end{proof}
It implies that
\begin{align*}
\| \Delta \partial^{\vnu}u\|_{L^2(D)} 
\leq
	\frac{2C_{\Delta} C_m^{-1} \,\tilde{\rho}^{|\vnu|}(|\vnu|!)^{\delta} }{\vR	^{\vnu}} .
\end{align*}

Finally we remark that $(\|u\|_{L^2(D)}^2 + \|\Delta u\|_{L^2(D)}^2)^{1/2}$ is an equivalent norm on $H^2(D) \cap H^1_0(D)$. Moreover, if $D$ is convex, the solution $u \in H^1_0(D)$ to \eqref{variational form} is in $H^2(D)$ by the  linear elliptic regularity theory, see e.g. \cite{Grisvard1985}. Indeed, the solution $u\in H^1_0(D)$ to \eqref{variational form} can be seen as the unique solution of
\[
\int_D a \nabla w \cdot \nabla v = \int_D \tilde f v, \qquad \forall v \in H^1_0(D),
\]
where $\tilde f := f - b u^m$. Since $H^1_0(D)$ is continuously embedded in $L^{2m}(D)$ and $\tilde f \in L^2(D)$, the linear elliptic regularity theory in convex domains applies. As a result we have in this case
\tl{\[
\|\partial^{\vnu} u\|_{H^2(D)} \lesssim (\|\partial^{\vnu}u\|_{L^2(D)}^2 + \|\Delta \partial^{\vnu} u\|_{L^2(D)}^2)^{1/2} \leq (((C_1C_u C_m^{-1})^2   +  (2C_\Delta C_m^{-1})^2)^{1/2} \frac{ (|\vnu|!)^{\delta}}{(\vR/\tilde \rho)^{\vnu}}.
\]}


==> Parametric_regularity_new.tex <==

\subsection{Parametric regularity in $H^1(D)$}

The following theorem is the first main regularity result of this paper.
\begin{theorem}\label{gevrey regularity for semilinear}
	Let the coefficients $a,b$ and the right-hand side $f$ of \eqref{variational form} satisfy Assumption \ref{Assumption} for some $\delta \geq 1$ and suppose moreover that either Assumption \ref{General b Assump} or Assumption \ref{Possitive b Assump} hold. Then the solution $u$ of \eqref{variational form} is of class Gevrey-$\delta$. More precisely, the following estimates are valid for all  $\vnu \in \newpart{\cF\setminus\sett{\vzero}}$ and $\vy \in U$
	\begin{align}\label{u V norm ref}
		\norm{\partial^{\vnu} u( \vy)}{V}
		\leq
		\frac{C_u \newpart{\rho^{\abs{\vnu}-1}} \gdnota{\abs{\vnu}}}{\vR^{{\vnu}}} (\abs{\vnu}!)^{\delta-1}
	\end{align}
	and
	\begin{align}\label{u H1 norm ref}
		\norm{\partial^{\vnu} u( \vy)}{H^1_0(D)}
		\leq
		\frac{C_u\newpart{\rho^{\abs{\vnu}-1}}(\abs{\vnu}!)^\delta }{C_m\vR^{\vnu}}.
	\end{align}
The constants in the above bounds are explicitly determined as 
\begin{equation} \label{Cu-rho-def}
C_u:=	\newpart{C_A^{-1}\overline{u}\brac{\overline{a}+\overline{b}\,\overline{u}^{m-1}+1}} \qquad \text{and} \qquad
\rho:=\newpart{ \max\sett{2,
\frac{2\overline{a}+\overline{b}\brac{m\overline{u}^{m-1}+ (3C_u)^{m-1}(m+1)}}{C_A}+1}}.
\end{equation}
\end{theorem}
To prove the above Theorem, we require auxiliary upper bounds for derivatives of the solution from Lemma \ref{lem:u-bnd} and Lemma \ref{upper bound for um derivative} below.
\begin{lemma}\label{lem:u-bnd}
	For sufficiently regular solutions of \eqref{semi prob} there holds
	\begin{equation}\label{u V norm upper}
		\begin{split}
			C_A\norm{\partial^{\vnu+\ve}u}{V}
			&\leq
			\newpart{\norm{\partial^{\vnu+\ve}a}{L^\infty(D)}
			\norm{u}{V}
+}
			\sum_{\newpart{\vzero< \veta\leq \vnu}}
			\brac{\vnu\atop \veta}
			\norm{\partial^{\vnu+\ve-\veta}a}{L^\infty(D)}
			\norm{\partial^{\veta}u}{V}
			\\
			&\quad			+\newpart{
			\norm{\partial^{\vnu+\ve}b}{L^\infty(D)}
			\norm{u^m}{\LL{m+1}{m}}}+
			\sum_{\newpart{\vzero< \veta\leq \vnu}}
			\brac{\vnu\atop \veta}
			\norm{\partial^{\vnu+\ve-\veta}b}{L^\infty(D)}
			\norm{\partial^{\veta}(u^m)}{\LL{m+1}{m}}\\
			&\quad+	\norm{\partial^{\vnu+\ve}f}{V^*}
			+
			\sum_{\vzero< \veta\leq \vnu}
			\brac{\vnu\atop \veta}
			\norm{\partial^{\veta}a}{L^\infty(D)}
			\norm{\partial^{\vnu+\ve-\veta}u}{V}\\
			&\quad\newpart{+
			m\sum_{\vzero< \veta\leq \vnu}
						\brac{\vnu\atop \veta}
			\norm{\partial^{\veta}b}{L^\infty(D)}
			\norm{u^{m-1}}{\LL{m+1}{m-1}}
			\| \partial^{\vnu+\ve-\veta} u\|_{\LL{m+1}{1}}}\\			
			&\quad+
			m\sum_{\vzero< \veta\leq \vnu}
			\sum_{\newpart{\vzero< \vell\leq \veta}}
						\brac{\vnu\atop \veta}
			\brac{\veta\atop \vell}
			\norm{\partial^{\veta-\vell}b}{L^\infty(D)}
			\norm{\partial^{\vell}(u^{m-1})}{\LL{m+1}{m-1}}
			\| \partial^{\vnu+\ve-\veta} u\|_{\LL{m+1}{1}},
		\end{split}
	\end{equation}
where $\ve$ is a unit \secondcmt{multi-index} in $\cF$, i.e. $\abs{\ve}=1$.
\end{lemma}
\begin{proof}
We recall the variational formulation \eqref{variational form} and take the $\ve$-th derivative \firstcmt{of both} sides with respect to $ \vy$. Collecting the terms with $\partial^{\ve} u$ on the left-hand side we obtain
	\begin{equation}\label{ve derivative}
		\begin{split}
			C_m^2\int_D a\, \partial^{\ve}\nabla u \cdot \nabla v 
			+
			m\int_D b\, u^{m-1} \partial^{\ve}u\, v
			=
			-
			C_m^2\int_D \partial^{\ve} a \nabla u\cdot\nabla v 
			-
			\int_D \partial^{\ve} b\, u^{m} v
			+		
				C_m\int_D \partial^{\ve} f v .
		\end{split}
	\end{equation}
Observe that the left-hand side can be expressed as $\wtd A_{\vy}(u,\partial^{\ve} u,v)$, where the linearized form $\wtd A_{\vy}$ has been introduced in \eqref{Atilde-def}. Notice that the first and the second argument of this expression depend on $\vy$. Therefore, if we take higher $\vnu$-th order derivatives of \eqref{ve derivative}, both the first and the second argument of $\wtd A_{\vy}$ will generate further terms by the Leibniz product rule. But the highest order derivative $\partial^{\vnu + \ve} u$ will only appear in the term $\wtd A_{\vy}(u,\partial^{\vnu+\ve} u,v)$. Isolating this term on the left-hand side, we obtain
\begin{equation}\label{vnu+ve derivative}
		\begin{split}
\wtd A_{\vy}(u,\partial^{\vnu+\ve} u,v)
		=&
		-
		C_m^2
		\sum_{\vzero\leq \veta\leq \vnu}
		\brac{\vnu\atop \veta}
		\int_D \partial^{\vnu+\ve-\veta} a\, \partial^{\veta}\nabla u\cdot\nabla v
		-
		\sum_{\vzero\leq \veta\leq \vnu}
		\brac{\vnu\atop \veta}
		\int_D \partial^{\vnu+\ve-\veta} b\, \partial^{\veta} (u^{m})  v+
		C_m\int_D \partial^{\vnu+\ve} f v \\
		&
		-
		C_m^2
		\sum_{\vzero< \veta\leq \vnu}
		\brac{\vnu\atop \veta}
		\int_D \partial^{\veta} a\, \partial^{\vnu+\ve-\veta}\nabla u\cdot\nabla v
		-
		m\sum_{\vzero< \veta\leq \vnu}
		\brac{\vnu\atop \veta}
		\sum_{\vzero\leq\vell\leq\veta}
		\brac{\veta\atop \vell}
		\int_D \partial^{\veta-\vell} b\, \partial^{\vell} (u^{m-1}) \partial^{\vnu+\ve-\veta} u\, v. 
	\end{split}
\end{equation}
Since \eqref{vnu+ve derivative} is valid for all $v \in V$ we may select specifically $v=\partial^{\vnu+\ve} u$. According to Lemma \ref{lem:coercive-type}, the left-hand side admits the bound $\wtd A_{\vy}(u,\partial^{\vnu+\ve} u,\partial^{\vnu+\ve} u)\geq C_{A} \norm{  \partial^{\vnu+\ve} u}{ V}^2$. Applying the triangle and the Cauchy-Schwarz inequality, we get the estimate
\begin{equation*}\label{vnu+ve derivative2}
		\begin{split}
C_{A} &\norm{  \partial^{\vnu+\ve} u}{V}
		\leq
		\sum_{\vzero\leq \veta\leq \vnu}
		\brac{\vnu\atop \veta}
		\|\partial^{\vnu+\ve-\veta} a\|_{L^\infty(D)}\, \|\partial^{\veta} u\|_V
		+
		\sum_{\vzero\leq \veta\leq \vnu}
		\brac{\vnu\atop \veta}
		\| \partial^{\vnu+\ve-\veta} b\|_{L^\infty(D)}\, \|\partial^{\veta} (u^{m})\|_{
		\LL{m+1}{m}
%		\cL_m
		}+
		\|\partial^{\vnu+\ve} f \|_{V^*} \\
		+&
		\sum_{\vzero< \veta\leq \vnu}
		\brac{\vnu\atop \veta}
		\| \partial^{\veta} a\|_{L^\infty(D)}\, \|\partial^{\vnu+\ve-\veta} u\|_V
		+
		m\sum_{\vzero< \veta\leq \vnu}
		\sum_{\vzero\leq\vell\leq\veta}
		\brac{\vnu\atop \veta}
		\brac{\veta\atop \vell}
		\|\partial^{\veta-\vell} b\|_{L^\infty(D)}\, \|\partial^{\vell} (u^{m-1})\|_{
		\LL{m+1}{m-1}
		%\cL_{m-1}
		} \, \| \partial^{\vnu+\ve-\veta} u\|_{
		\LL{m+1}{1}}	,
	\end{split}
\end{equation*}
where we have applied the H\"older inequality \eqref{adjusted Hoelder} and the Sobolev embedding estimate \eqref{Sobolev ineq} for the terms on the right-hand side. Notice that $\|\partial^{\vnu+\ve} u\|_V$ is cancelled on the both sides. \newpart{We conclude the proof by separating the terms with $\veta=\vzero$ in the first two sums and the term with $\vell=\veta$ in the last sum.}
%Finally, observe that the Sobolev embedding also yields $\norm{\partial^{\vnu+\ve-\veta}u}{\LL{m+1}{1}} = \|\partial^{\vnu+\ve-\veta}u\|_{L^{m+1}(D)}\leq \norm{\partial^{\vnu+\ve-\veta}u}{\V}$ and, hence, the statement of the Lemma.
\end{proof}	
\newpart{\begin{remark}
The existence and uniqueness of the partial derivatives $\partial^{\vnu+\ve}u$ at some $\vy\in U$ for all $\vnu\in\cF$ follows by induction. Indeed, for the inductive step, the equation \eqref{vnu+ve derivative} illustrates that $\partial^{\vnu+\ve}u$ is determined by its lower order derivatives. Thus, when combined with Lemma \ref{lem:coercive-type}, it confirms the well-posedness of $\partial^{\vnu+\ve}u$.
\end{remark}}
The right-hand side of \eqref{u V norm upper} contains the terms of the type $\norm{\partial^{\vmu}(u^k)}{\LL{m+1}{k}}$, where $k = m-1$ or $m$ and $\vmu \in \newpart{\cF\setminus\sett{\vzero}}$. The following result is a corollary of the general Lemma \ref{upper bound for f derivative} and determines explicit upper bounds for these powers of $u$, if corresponding bounds for $u$ are available. This result together with Lemma \ref{lem:u-bnd} is the key ingredient in the inductive proof of Theorem \ref{gevrey regularity for semilinear}.
\begin{corollary}\label{upper bound for um derivative}
	Let \newpart{$u(\vy)\in\cB(0,\overline{u})$ and} $\vmu\in \newpart{\cF\setminus\sett{{\vzero}}}$, suppose that \eqref{u V norm ref} holds for all multi-index \newpart{$\vell\in \cF\setminus\sett{{\vzero}}$ and} $\vell\leq \vmu$, i.e.
	\begin{align}\label{uV deri}
		\norm{\partial^{\vell} u (\vy)}{V}
		\leq
		\frac{C_u \rho^{\abs{\vell}-1} \gdnota{\abs{\vell}}}{\vR^{{\vell}}} (\abs{\vell}!)^{\delta-1} \newpart{\qall \vell \leq \vmu \text{ and } \abs{\vell}\geq 1}.
	\end{align}
Then, for all positive integers $q\leq m+1$ the following estimates are valid
	\begin{equation} \label{um derivative}
		\norm{\partial^{\vmu}(u(\vy)^q)}{\LL{m+1}{q}}
		\leq
		\frac{(\newpart{3}^{q-1}C_u^{q})\, \rho^{\newpart{\abs{\vmu}-1}} \gdnota{\abs{\vmu}}}{\vR^{{\vmu}}}
		(\abs{\vmu}!)^{\delta-1}
	\end{equation}
	as long as $(d,m) \in \cM$, i.e. $H^1(D)$ is continuously embedded into $L^{m+1}(D)$.
\end{corollary}
\begin{proof}
\newpart{Notice that $\overline{u}\leq C_u$, we have $u(\vy)\in\cB(0,\overline{u})\subset\cB(0,C_u)$. We also notice definition of $\rho$ in \eqref{Cu-rho-def} then $\rho\geq 2$.} If $(d,m) \in \cM$, we have $\|u\|_{L^{m+1}(D)} \leq \|u\|_V$ and therefore the statement of the lemma follows immediately from Lemma \ref{upper bound for f derivative} with \newpart{$C_u$, $\rho$ and $\vR/\rho$} in place of \newpart{$C_f$, $\rho$ and $\vR$} respectively.
\end{proof}
\begin{proof}[Proof of Theorem \ref{gevrey regularity for semilinear}]
Observe that \eqref{u H1 norm ref} is a simple corollary from \eqref{u V norm ref} by changing from the $V$-norm to the $H^1_0(D)$-norm and the trivial bound $\gdnota{n}\leq n!$. Therefore it remains to prove \eqref{u V norm ref}. Here we argue by induction with respect to the order of the derivative $\vnu$. For the first-order derivatives we use \eqref{u V norm upper} with $\vnu = \vzero$ and get
\begin{align*}
	C_A\norm{\partial^{\ve}u}{V}
	\leq
	\norm{\partial^{\ve} a}{L^\infty(D)}\norm{u}{V}
	+
	\norm{\partial^{\ve} b}{L^\infty(D)}\norm{u^m}{\LL{m+1}{m}}
	+
	\norm{\partial^{\ve} f}{V^*}.
\end{align*} 
For the term with $u^m$ we recall the H\"older estimate \eqref{multiple Hoelder}, the Sobolev embedding \eqref{Sobolev ineq}, and \eqref{u-bound} to obtain the upper bound $\norm{u^m}{\LL{m+1}{m}} \leq \norm{u}{\LL{m+1}{1}}^m \leq \|u\|_V^m\leq \overline{u}^m$. Using this and the regularity assumption \eqref{abf assumption}, we derive
\begin{align*}
	\norm{\partial^{\ve}u}{V}
	\leq
	\frac{\overline{a} \gdnota{1}}{C_A\vR^{\ve}}  \, \overline{u}
	+
	\frac{\overline{b} \gdnota{1}}{C_A\vR^{\ve}}  \, \overline{u}^m
	+
	\frac{\overline{f} \gdnota{1}}{C_A\vR^{\ve}} 
	=
	\overline{u}\brac{\overline{a}+\overline{b}\,\overline{u}^{m-1}+1}
	\frac{\gdnota{1}}{C_A\vR^{\ve}}
	\leq C_u \frac{\gdnota{1}}{\vR^{\ve}}.
\end{align*}
Thus, the base of induction is satisfied for the constant $C_u$ defined in \eqref{Cu-rho-def}. 
Suppose now that \eqref{u V norm ref} is valid for the $\vnu$-th derivative. Our aim is to show that the same bound holds for the $(\vnu + \ve)$-th order derivative, where $\abs{\vnu}\geq 1$ and $\ve$ is a unit \secondcmt{multi-index}. 
For this we combine \eqref{u V norm upper} with regularity assumptions \eqref{abf assumption}, the inductive assumption, and \eqref{um derivative} for $\vmu \leq \vnu$ (this is valid by Corollary \ref{upper bound for um derivative} and the inductive assumption) to arrive at

\begin{align*}
	C_A\norm{\partial^{\vnu+\ve}u}{V}
&\leq
\newpart{\frac{\overline{u}\,\overline{a} \gdnota{\abs{\vnu+\ve}}}{\vR^{\vnu+\ve}}(\abs{\vnu+\ve}!)^{\delta-1}
+
}\sum_{\newpart{\vzero< \veta\leq \vnu}}
\brac{\vnu\atop \veta}
\frac{\overline{a} \gdnota{\abs{\vnu+\ve-\veta}}}{\vR^{\vnu+\ve-\veta}}(\abs{\vnu+\ve-\veta}!)^{\delta-1}\,
\frac{C_u \rho^{\newpart{\abs{\veta}-1}} \gdnota{\abs{\veta}}}{\vR^{{\veta}}}
(\abs{\veta}!)^{\delta-1}\\
&\quad\newpart{+
\frac{\overline{u}^{m}\overline{b} \gdnota{\abs{\vnu+\ve}}}{\vR^{\vnu+\ve}}(\abs{\vnu+\ve}!)^{\delta-1}
}+
\sum_{\newpart{\vzero<\veta\leq \vnu}}
\brac{\vnu\atop \veta}
\frac{\overline{b} \gdnota{\abs{\vnu+\ve-\veta}}}{\vR^{\vnu+\ve-\veta}}(\abs{\vnu+\ve-\veta}!)^{\delta-1}\,
\frac{\newpart{3}^{m-1}C_u^{m} \,\rho^{\newpart{\abs{\veta}-1}} \gdnota{\abs{\veta}}}{\vR^{{\veta}}}(\abs{\veta}!)^{\delta-1}
\\
&\quad+	
\frac{\overline{f} \gdnota{\abs{\vnu+\ve}}}{\vR^{\vnu+\ve}} (\abs{\vnu+\ve}!)^{\delta-1}
+
\sum_{\vzero< \veta\leq \vnu}
\brac{\vnu\atop \veta}
\frac{\overline{a} \gdnota{\abs{\veta}}}{\vR^{\veta}}(\abs{\veta}!)^{\delta-1}\,
\frac{C_u \rho^{\newpart{\abs{\vnu+\ve-\veta}-1}} \gdnota{\abs{\vnu+\ve-\veta}}}{\vR^{{\vnu+\ve-\veta}}}(\abs{\vnu+\ve-\veta}!)^{\delta-1}
\\
&\quad\newpart{+
m\sum_{\vzero< \veta\leq \vnu}
\brac{\vnu\atop \veta}
\frac{\overline{u}^{m-1}\overline{b} \gdnota{\abs{\veta}}}{\vR^{\veta}}(\abs{\veta}!)^{\delta-1}
\frac{C_u\, \rho^{\abs{\vnu+\ve-\veta}-1}
	\gdnota{\abs{\vnu+\ve-\veta}}}{\vR^{{\vnu+\ve-\veta}}}(\abs{\vnu+\ve-\veta}!)^{\delta-1}}
\\
&\quad+
m\sum_{\vzero< \veta\leq \vnu}
\sum_{\newpart{\vzero< \vell \leq \veta}}
\brac{\vnu\atop \veta}\brac{\veta\atop \vell}
\frac{\overline{b} \gdnota{\abs{\veta-\vell}}}{\vR^{\veta-\vell}\, (\abs{\veta-\vell}!)^{1-\delta}}\,
\frac{\newpart{3}^{m-2} {C_u}^{m-1}\,\rho^{\newpart{\abs{\vell}-1}} \gdnota{\abs{\vell}}}{\vR^{{\vell}}\, (\abs{\vell}!)^{1-\delta}}
\frac{C_u\, \rho^{\newpart{\abs{\vnu+\ve-\veta}-1}}
	\gdnota{\abs{\vnu+\ve-\veta}}}{\vR^{{\vnu+\ve-\veta}}\,(\abs{\vnu+\ve-\veta}!)^{1-\delta}}.
\end{align*}
Bound \eqref{multiindex-est-1} yields estimates for products of the factorial terms. Observe that $0 < C_A \leq 1$ and therefore $\rho \geq 2$. This helps to extract common factors on the right-hand side and obtain
\begin{align*}
	C_A\norm{\partial^{\vnu+\ve}u}{V}
	&\leq
	\frac{\rho^{\newpart{\abs{\vnu}-1}}(\abs{\vnu+\ve}!)^{\delta-1}}{ \vR^{\vnu+\ve}}
	\bigg(
\newpart{\overline{u}\, \overline{a}\gdnota{\abs{\vnu+\ve}}+}C_u \, \overline{a} 
	\sum_{\newpart{\vzero< \veta\leq \vnu}}
	\brac{\vnu\atop \veta}
	\gdnota{\abs{\vnu+\ve-\veta}}
	  \gdnota{\abs{\veta}} \\
	&\quad+
\newpart{\overline{u}^m\, \overline{b}\gdnota{\abs{\vnu+\ve}}}+
	\newpart{3}^{m-1} C_u^m 
\overline{b}\,
	\sum_{\newpart{\vzero< \veta\leq \vnu}}
	\brac{\vnu\atop \veta}
	\gdnota{\abs{\vnu+\ve-\veta}}
	\gdnota{\abs{\veta}}
	+	
	 \overline{f}\gdnota{\abs{\vnu+\ve}}\\
		&\quad
	+
	\overline{a}C_u  
	\sum_{\vzero< \veta\leq \vnu}
	\brac{\vnu\atop \veta}
	\gdnota{\abs{\vnu+\ve-\veta}}
	\gdnota{\abs{\veta}} 
\newpart{+m\,\overline{u}^{m-1}C_u\,
\overline{b}
	\sum_{\vzero< \veta\leq \vnu}
	\brac{\vnu\atop \veta}
		\gdnota{\abs{\vnu+\ve-\veta}}
	\gdnota{\abs{\veta}}}
	\\
	&\quad+
	\newpart{m}\,\newpart{3}^{m-2}C_u^{m}\overline{b}\,
	\sum_{\vzero< \veta\leq \vnu}
	\sum_{\newpart{\vzero< \vell\leq \veta}}
	\brac{\vnu\atop \veta}\brac{\veta\atop \vell}
	\gdnota{\abs{\veta-\vell}}
	\gdnota{\abs{\vell}}
		\gdnota{\abs{\vnu+\ve-\veta}} \bigg).
\end{align*}
According to \eqref{multiindex-est-6} and \eqref{multiindex-est-5}, the bound for \firstcmt{the} first four sums is $[\tfrac{1}{2}]_{|\vnu+\ve|}$, the last sum bounded by $\newpart{3} [\tfrac{1}{2}]_{|\vnu+\ve|}$. Recalling that $\overline{f} \leq \overline{u}$  we arrive at
\begin{align*}
	\norm{\partial^{\vnu+\ve}u}{V}&\leq
	\newpart{\frac{\overline{u}\brac{\overline{a}+\overline{b}\,\overline{u}^{m-1}+1}+
2\overline{a}C_u
+
m\overline{b} \,\overline{u}^{m-1} C_u
		+
	\overline{b}C_u^{m}
\brac{3^{m-1}+3m\,3^{m-2}}
		}{C_u	C_A}}\,
\frac{	\newpart{C_u}\,\rho^{\abs{\vnu}-1}(\abs{\vnu+\ve}!)^{\delta-1}}{\vR^{\vnu+\ve}}
		\gdnota{\abs{\vnu+\ve}}\\
		&
		\leq
		\frac{		C_u\,\rho^{\newpart{\abs{\vnu}}}(\abs{\vnu+\ve}!)^{\delta-1}}{\vR^{\vnu+\ve}}
		\gdnota{\abs{\vnu+\ve}},
\end{align*}
where we have used the definition \eqref{Cu-rho-def} of $\rho$ in the last step.
\secondcmt{This} completes the inductive argument and thereby the proof of the theorem.
\end{proof}

\subsection{Parametric regularity in $H^2(D)$ and pointwise estimates}

If $D$ is a convex Lipschitz domain and the coefficients $a,b$ and the right-hand side $f$ are sufficiently regular, it is actually possible to prove that estimates of the type \eqref{u H1 norm ref} remain valid in $H^2(D)$, and therefore in every space containing $H^2(D)$ with continuous embedding. In particular, pointwise estimates follow from $L^\infty(D)$ bounds. 

If the data are sufficiently regular (see Assumption \ref{Assumption1} below for the precise regularity assumptions), formal  
integration by parts in the variational formulation \eqref{variational form} delivers
\begin{equation*}
\firstcmt{C_m^2 a \Delta u = b u^m - C_m^2\nabla a \cdot \nabla u - C_m f.}
\end{equation*}
\firstcmt{Since the right hand side belong to $L^2(D)$, it shows that $\Delta u\in L^2(D)$.} The Leibniz product rule implies
\begin{equation}\label{Delta u variational form}
\firstcmt{ C_m^2 a (\Delta \partial^{\vnu} u) =  \partial^{\vnu}(b u^m - C_m^2\nabla a \cdot \nabla u -  C_mf) -
C_m^2\sum_{\vzero \leq \veta < \vnu }
\binom{\vnu}{\veta} \partial^{\vnu-\veta} a (\Delta \partial^{\veta} u).}
\end{equation}
\firstcmt{The recurrent equation above implies that we can determine $\Delta \partial^{\vnu} u$ based on $\Delta \partial^{\veta} u$ with $\eta<\vnu$, thereby ensuring that $\Delta \partial^{\vnu} u \in L^2(D)$. Apply the triangle and the Cauchy-Schwarz inequalities and recall that $a\geq 1$, and hence}
\begin{equation}\label{vnu-Delta-u}
C_m^2\|\Delta \partial^{\vnu} u\|_{L^2(D)}
\firstcmt{\leq
\|C_m^2 a (\Delta \partial^{\vnu} u)\|_{L^2(D)}}
\leq \|\partial^{\vnu} ( b u^m - C_m^2\nabla a \cdot \nabla u - C_m f)\|_{L^2(D)} 
+ C_m^2\sum_{\vzero \leq \veta < \vnu }
\binom{\vnu}{\veta} \|\partial^{\vnu-\veta} a\|_{L^\infty(D)} \|\Delta \partial^{\veta} u\|_{L^2(D)}.
\end{equation}
The second term admits Gevrey-$\delta$ bounds if $L^\infty(D)$ and $V^*$-norms for $a$ and $f$ in Assumption \ref{Assumption} are replaced by the $W^{1,\infty}(D)$ and $L^2(D)$-norms respectively. More precisely, we replace Assumption \ref{Assumption} by the following.
	\begin{assumption} \label{Assumption1}
		For all fixed values $\vy\in U \in \mR^s$ with $s<\infty$, the coefficients $a(\vy) \in W^{1,\infty}(D)$, $b(\vy) \in L^\infty(D)$ and $f(y)\in L^2(D)$. Moreover, for all $\vnu\in \mN^s$ there exist positive constants $\vR=(R_1,R_2,\dots)$ independent of $s$ such that
		\begin{align*}
			\norm{\partial^{\vnu} a(\vy)}{W^{1,\infty}(D)}
			\leq
			\frac{\overline{a}}{2}
			\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}} , \qquad
			\norm{\partial^{\vnu} b(\vy)}{L^\infty(D)}
			\leq
			\frac{\overline{b}}{2}
			\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}} , \qquad
			\norm{\partial^{\vnu} f(\vy)}{L^2(D)}
			\leq
			\frac{\overline{f}}{2}
			\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}}  .
		\end{align*} 
Assume moreover, that $m \in \mN$ is such that $H^1(D)$ is continuously embedded into $L^{2m}(D)$, i.e. $(d,2m-1) \in \cM$, see \eqref{cond: m d restriction}.
	\end{assumption}
According to \eqref{ff-estimates} Assumption \ref{Assumption1} implies
\begin{align}\label{abf1 assumption}
	\norm{\partial^{\vnu} a(\vy)}{W^{1,\infty}(D)}
	\leq
	\frac{\overline{a} \gdnota{\abs{\vnu}}}{\vR^{\vnu}} (\abs{\vnu}!)^{\delta-1} , \qquad
	\norm{\partial^{\vnu} b(\vy)}{L^\infty(D)}
	\leq
	\frac{\overline{b} \gdnota{\abs{\vnu}}}{\vR^{\vnu}}
	(\abs{\vnu}!)^{\delta-1} , \qquad
	\norm{\partial^{\vnu} f(\vy)}{L^2(D)}
	\leq
	\frac{\overline{f} \gdnota{\abs{\vnu}}}{\vR^{\vnu}}(\abs{\vnu}!)^{\delta-1}.
\end{align}
 The regularity of $\Delta \partial^{\vnu} u$ can now be established by bounding the terms in the right-hand side of \eqref{vnu-Delta-u}. Indeed, for $\vnu=\vzero$, we choose $v=\Delta u$ in \eqref{Delta u variational form} to derive
\begin{align}\label{C_delta}
C_m^2\|\Delta u\|_{L^2(D)}
&\leq
\|b u^m - C_m^2\nabla a \cdot \nabla u - C_m\,f\|_{L^2(D)}
\leq
\norm{b}{L^{\infty}(D)}
\norm{u^m}{L^2(D)}
+
C_m^2
\norm{\nabla a}{L^{\infty}(D)}
\norm{\nabla u}{L^2(D)}
+
C_m
\norm{f}{L^2(D)}\notag\\
&\leq
\frac{1}{2}
\brac{
\overline{b}
(C_m^{-1}\overline{u})^m
+
C_m
\overline{a}\,
\overline{u}
+
C_m \overline{f}}.
\end{align} 
For all $\vnu\in \cF\setminus\sett{\vzero}$, the Leibniz general product rule and the triangle inequality yield for the first term of \eqref{vnu-Delta-u}
\begin{equation}\label{term-1}
\begin{split}
\|\partial^{\vnu} &(b u^m - C_m^2\nabla a \cdot \nabla u - C_m\,f)\|_{L^2(D)}\\
&\leq 
C_m \|\partial^{\vnu} f\|_{L^2(D)}
+
\sum_{\vzero \leq \veta \leq \vnu} \binom{\vnu}{\veta}
\big(
\|\partial^{\vnu-\veta} b\|_{L^\infty(D)} \|\partial^{\veta} (u^m)\|_{L^2(D)}
+ C_m^2\|\partial^{\vnu-\veta} \nabla  a\|_{L^\infty(D)} \|\partial^{\veta}\nabla  u\|_{L^2(D)}
\big)\\
&\leq 
C_m\|\partial^{\vnu} f\|_{L^2(D)}
\newpart{+
\|\partial^{\vnu} b\|_{L^\infty(D)} \|u^m\|_{L^2(D)}
+
C_m^2\|\partial^{\vnu} \nabla  a\|_{L^\infty(D)} \|\nabla  u\|_{L^2(D)}}
\\&\quad+
\frac{(|\vnu|!)^{\delta-1}}{\vR^{\vnu}}
\sum_{\newpart{\vzero < \veta \leq \vnu}} \binom{\vnu}{\veta}
\big(
3^{m-1} (C_{2m-1} C_m^{-1}  C_u)^m \overline{b} +  C_m C_u \overline{a}
\big) \rho^{|\veta|-1} \gdnota{|\vnu-\veta|} \gdnota{|\veta|}\\
&\leq 
\big(
\newpart{\overline{b}\,(C_m^{-1}\overline{u})^{m}
+
C_m \overline{a}\, \overline{u}
+}
\newpart{3}^m(C_{2m-1} C_m^{-1}  C_u)^m \overline{b}  + \newpart{3}C_m C_u \overline{a}
+C_m\overline{f}
\big)
\frac{  \rho^{|\vnu|-1} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1},
\end{split}
\end{equation}
In the above estimate we used \eqref{multiindex-est-3} and that the \newpart{following bounds hold for all $\veta\in\cF\setminus\sett{\vzero} $}
\begin{equation*}
\|\partial^{\veta} u\|_{L^{2m}(D)} 
\leq C_{2m-1}
\|\partial^{\veta} u\|_{H^1_0(D)} 
= C_{2m-1} C_m^{-1}
\|\partial^{\veta} u\|_V
\leq C_{2m-1} C_m^{-1}  C_u 
\frac{ \rho^{\newpart{|\veta|-1}} \gdnota{|\veta|} }{\vR^{\veta}}(|\veta|!)^{\delta-1},
\end{equation*}
i.e. the Sobolev embedding for $(d,2m-1) \in \cM$, and Theorem \ref{gevrey regularity for semilinear}. By Lemma \ref{upper bound for f derivative} this implies
\begin{equation*}
\|\partial^{\veta} (u^m)\|_{L^2(D)} 
=
\|\partial^{\veta} (u^m)\|_{\LL{2m}{m}} 
\leq 
\newpart{3}^{m-1} (C_{2m-1} C_m^{-1}  C_u)^m\,
\frac{ \rho^{\newpart{|\veta|-1}} \gdnota{|\veta|} }{\vR^{\veta}}(|\veta|!)^{\delta-1}
\end{equation*}
and hence \eqref{term-1}.
The argument can now be completed by induction, which is the subject of the following Theorem.
\begin{theorem}\label{thm:2}
Suppose the assumptions of Theorem \ref{gevrey regularity for semilinear} hold and additionally Assumption \ref{Assumption1} is satisfied. Then $\Delta \partial^{\vnu} u \in L^2(D)$  for all \newpart{$\vnu \in \cF\setminus\sett{\vzero}$} and there holds
\begin{equation}\label{Delta-u-derivative}
C_m^2\|\partial^{\vnu}\Delta u\|_{L^2(D)} \leq 
\frac{2 {C}_{\Delta} \tilde{\rho}^{|\vnu|-1} \gdnota{|\vnu|}}{\vR	^{\vnu}} (|\vnu|!)^{\delta-1},
\end{equation}
where $\tilde \rho := \max(4\overline{a},\rho)$ and
\begin{align*}
\newpart{C_{\Delta} =
\brac{\brac{1+\frac{\overline{a}}{2}}\brac{C_m\overline{f}
+
\overline{b}\,(C_m^{-1}\overline{u})^{m}
+
C_m \overline{a}\, \overline{u}}
+
(3C_{2m-1} C_m^{-1}  C_u)^m \overline{b}  + 3C_m C_u \overline{a}
}.
}
\end{align*}
\end{theorem}
\begin{proof}
We prove the statement by induction. For $\vnu = \ve$ we have by \eqref{C_delta} and \eqref{term-1}
\begin{equation*}
\newpart{\begin{split}
C_m^{2}\|\partial^{\ve}\Delta u\|_{L^2(D)} 
&\leq  \| \partial^{\ve}( bu^m - C_m^2\nabla a \cdot \nabla u - C_m f)\|_{L^2(D)}
+
\norm{\partial^{\ve}\nabla a}{L^{\infty}(D)}C_m^2 \norm{\Delta u}{L^2(D)}\\
&\leq \big(
\overline{b}\,(C_m^{-1}\overline{u})^{m}
+
C_m \overline{a}\, \overline{u}
+
(3C_{2m-1} C_m^{-1}  C_u)^m \overline{b}  + 3C_m C_u \overline{a}
+C_m\overline{f}
\big)
\frac{  \gdnota{1} }{\vR^{\ve}}
\\&\quad
+
\frac{1}{2}\big(
C_m\overline{f}
+
\overline{b}\,(C_m^{-1}\overline{u})^{m}
+
C_m \overline{a}\, \overline{u}\big)
\frac{  \overline{a}\gdnota{1} }{\vR^{\ve}}
=
 {C}_{\Delta}\frac{ \gdnota{1} }{\vR^{\ve}}
\leq 2 {C}_{\Delta}\frac{ \gdnota{1} }{\vR^{\ve}}.
\end{split}}
\end{equation*}
The aim is now to prove \eqref{Delta-u-derivative}, assuming that it is valid for all derivatives of order strictly less than $\vnu$. From \eqref{vnu-Delta-u} and the bound below it, we readily have for $|\vnu|\geq 2$
\begin{equation*}
\begin{split}
C_m^2 \|\partial^{\vnu}  \Delta u\|_{L^2(D)}
&\newpart{\leq 
\|\partial^{\vnu} (b u^m - C_m^2\nabla a \cdot \nabla u - C_m\,f)\|_{L^2(D)}
+
 \|\partial^{\vnu}\nabla a\|_{L^\infty(D)} 
C_m^2 \|\Delta u\|_{L^2(D)}}\\
&\quad\newpart{+
\sum_{\vzero < \veta < \vnu }
\binom{\vnu}{\veta} \|\partial^{\vnu-\veta}\nabla a\|_{L^\infty(D)} 
C_m^2 \|\partial^{\veta}\Delta  u\|_{L^2(D)}}\\
&\leq 
C_\Delta
\frac{  \rho^{\newpart{|\vnu|-1}} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1} +
\sum_{\newpart{\vzero < \veta < \vnu} }
\binom{\vnu}{\veta} 
\frac{\overline{a}\gdnota{|\vnu-\veta|}}{\vR^{\vnu-\veta}} (|\vnu-\veta|!)^{\delta-1} 
\frac{2{C}_\Delta \tilde{\rho}^{\newpart{|\veta|-1}}\gdnota{|\veta|}}{\vR^{\veta}} (|\veta|!)^{\delta-1} \\
&\leq 
2 {C}_\Delta
\frac{  \tilde \rho^{\newpart{|\vnu|-1}} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1} \big(\frac{1}{2} + \frac{\newpart{2}\overline{a}}{\tilde \rho}\big).
\end{split}
\end{equation*}
According to the definition of $\tilde \rho$ the term in the  parentheses is bounded by 1 and the claim of the theorem follows.
\end{proof}

Finally we remark that $(\|u\|_{L^2(D)}^2 + \|\Delta u\|_{L^2(D)}^2)^{1/2}$ is an equivalent norm on $H^2(D) \cap H^1_0(D)$. Moreover, if $D$ is convex, the solution $u \in H^1_0(D)$ to \eqref{variational form} is in $H^2(D)$ by the  linear elliptic regularity theory, see e.g. \cite{Grisvard1985}. Indeed, the solution $u\in H^1_0(D)$ to \eqref{variational form} can be seen as the unique solution of
\[
\int_D a \nabla w \cdot \nabla v = \int_D \tilde f v, \qquad \forall v \in H^1_0(D),
\]
where $\tilde f := C_m^{-1} f - C_m^{-2} b u^m$. Since $H^1_0(D)$ is continuously embedded in $L^{2m}(D)$ and $\tilde f \in L^2(D)$, the linear elliptic regularity theory in convex domains applies. Recalling \eqref{ff-estimates}, \newpart{for all $\vnu\in \cF\setminus\sett{\vzero}$} we have as a result in this case
\[
\|\partial^{\vnu}u\|_{H^2(D)} \lesssim (\|\partial^{\vnu}u\|_{L^2(D)}^2 + \|\Delta \partial^{\vnu} u\|_{L^2(D)}^2)^{1/2} \leq ((C_1C_m^{-1}C_u)^2  +  (2 C_m^{-2} C_\Delta )^2)^{1/2} \frac{ (|\vnu|!)^{\delta}}{(\vR/\tilde \rho)^{\vnu}},
\]
\newpart{where $C_1$ is the constant of Sobolev embedding $H^1_0(D)\hookrightarrow L^2(D)$, i.e. $\norm{v}{L^2(D)}\leq C_1 \norm{ \nabla v}{L^2(D)}$.}


==> QMC2.tex <==
In this section we give an example for the case of high-dimensional parametric integration and demonstrate an application of Theorem \ref{thm:2}. For this, we consider the variational problem \eqref{variational form} with $s$ parameters $\vy = (y_1,\dots,y_s)$ and the quantity of interest being the integral
\begin{align}\label{approx integral}
	I_s(\newpart{F}) =	
	\int_{U} \newpart{F}(\vy) \, d y_1 \dots dy_s,
\end{align}
where the functional $\newpart{F}(\vy):=u(\vx_0, \vy)$ is the point-evaluation of the solution $u$ in the middle of the computational domain $D= (0,1)^2$ and the $s$-dimensional unit cube $U = [-\frac{1}{2},  \frac{1}{2}]^s$ is the parameter domain. Such problems arise when the coefficients of \eqref{variational form} are modelled as general random fields e.g. via their Karhunen-L\`oeve expansion \cite{HansenSchwab13,CohenDevoreSchwab2011,KuoSchwabSloan2013,KuoSchwabSloan2012} and then truncated to a certain dimension $s$ for computational reasons. For further comments on the analysis of the truncation error for Gevrey-class parametrizations we refer to \cite[Section 6.2]{ChernovLe2023} and further references therein.


%To show the wide application range of our main regularity result, we now present a numerical experiment on the performance of Quasi-Monte Carlo (QMC) method. There is high demand for integration of functions of infinitely many variables as following
%
%where $Y=\left[-\frac{1}{2},  \frac{1}{2}\right]$. The function $F(\vy) := \cG(u(\vy))=u(\vx_0,\vy)$, is the point evaluation at the center of the computational domain $D$, i.e. the same linear functional introduced in Section \ref{sec: Gauss-Legendre Quadrature}. 
%We denote by $s\in \mN$ the dimensional truncation parameter and $\vy_s= (y_1,\dots,y_s,0,0,\dots) $ the $s$-dimensional truncation of $\vy\in U=Y^{\mN}$. In this section, our quantity of interest is a truncation of $I(F)$ of the form
%\begin{align}
%I_s(F) =	
%\int_{Y^s} F({\vy}_s)\, d y_1 \dots d y_s.
%\end{align}
%\tl{To guarantee the truncation error $|I(F)-I_s(F)|$ converges when $s\goto \infty$}, we propose a sufficient condition on the given data as below
%	\begin{align}\label{beta-lp}
%		\norm{\vbeta}{\ell^p}:= \bigg(\sum_{j = 1}^\infty \beta_j^{p}\bigg)^{\frac{1}{p}} < \infty
%	\end{align}
%for some $p \in (0,1]$ and $\beta_j:= \abs{\partial_{j} F}$, i.e. the bound for $j$-th derivative $\abs{\partial_j F}$ \tl{goes to zero with faster rate than $j$ does}.
%The truncation error $|I(F)-I_s(F)|$ has been intensively discussed in \cite[Theorem 4.3]{GuthKaarnioja2023} and \cite[Lemma 7.3]{ChernovLe2023}. 

In this section we fix the dimension of the parameter domain at $s = 100$ and concentrate on estimation of $I_s(u)$ where $u$ is a solution for the variational formulation \eqref{variational form} with $a\equiv 1$, $f\equiv 1$, the reaction coefficient $b$ being one of following functions
\begin{equation}\label{QMC-a1-new}
	b^{(1)} (\vx,\vy) = 
	2+2\exp\brac{-{\zeta(5)}+\sum_{j=1}^{s}
		{j^{-5}}
		 \sin(j\pi  x_1)\sin(j\pi x_2)\,y_j},
\end{equation}
or
\begin{equation}\label{QMC-a2-new}
	b^{(2)} (\vx,\vy) = 3+\frac{1}{\zeta(5)} \sum_{j=1}^{s} j^{-5} \sin(j\pi  x_1)\sin(j\pi x_2)\exp\brac{
		-\frac{1}{y_j+\tfrac{1}{2}}}.
\end{equation}
Here $y_j$ are independent uniformly distributed in $[-\frac{1}{2},\frac{1}{2}]$ random variables for all $1 \leq j\leq s$. Notice that $b^{(1)}$ is analytic with respect to $\vy$ ($\delta^{(1)} = 1$), whereas $b^{(2)}$ is of Gevrey-$\delta$ class with $\delta^{(2)} = 2$, \firstcmt{i.e. $ b^{(1)} \in G^1(U,L^{\infty}(D))$ and $ b^{(2)} \in G^2(U,L^{\infty}(D))$}. Notice also that both $b^{(1)}$ and $b^{(2)}$ are $\ell^p$-summable with $p$ less than one. More precisely, with any $p > \frac{1}{5}$. This will be important for the convergence of the Quasi-Monte-Carlo \newpart{(QMC)} methods, as explained below.

Theorem \ref{gevrey regularity for semilinear} and Theorem \ref{thm:2} imply that $\newpart{F}(\vy)$ is Gevrey-$\delta$ regular with the same $\delta$ as for $b^{(1)}$ and $b^{(2)}$. This follows since $H^2(D)$ is continuously embedded in $L^\infty(D)$ and $(\|u\|_{L^2(D)}^2 + \|\Delta u\|_{L^2(D)}^2 )^{1/2}$ is an equivalent norm on $H^2(D)$.


The quantity of interest for the coefficient $b^{(k)}$ will be denoted by $I_s(\newpart{F}^{(k)})$, $k = 1,2$. The standard Monte Carlo \newpart{(MC)} quadrature is the sample mean approximation $Q^{MC}_{s,n}(\newpart{F}) := \frac{1}{n} \sum_{i=1}^n \newpart{F}(\vy_s^{(i)})$, where $\vy_s^{(i)}$ are independent samples uniformly distributed in $U$. It satisfies the classical error estimate for the relative root mean square error
\begin{equation}\label{errorMC}
	\varepsilon^{\textrm{MC},(k)}_n := \sqrt{\mE\brac{ \abs{\frac{I_s(\newpart{F}^{(k)})-Q^{MC}_{s,n}(\newpart{F}^{(k)})}{I_s(\newpart{F}^{(k)})}}^2}}
	\lesssim C n^{-\frac{1}{2}}
\end{equation}
for a positive constant $C$ independent of $n$.
Observe that the asymptotic error bound is insensitive to the Gevrey class regularity of $\newpart{F}$. As an alternative to the standard \newpart{(MC)} quadrature, we consider a class of \newpart{QMC} rules called randomly shifted rank-1 lattice rules defined as
\begin{align}\label{QMC quad def}
	Q^{\Delta}_{s,n}(\newpart{F}) := 
	\frac{1}{n} \sum_{i=1}^n \newpart{F}\big(\left\{ \tfrac{i \vz_{s}}{n} +\Delta  \right\} -\tfrac{1}{2}\big).
\end{align}
Here the braces in \eqref{QMC quad def} indicate the fractional part of each component of the argument vector, see for e.g. \cite{KuoNuyens2016}, \cite{KuoSchwabSloan2012}. The quadrature points are constructed using a generating vector $\vz_{s} \in \mN^s$, and a random shift $\Delta$, which is a random variable uniformly distributed over the cube $(0,1)^s$. 
Since $Q^{\Delta}_{s,n}(G)$ is also a random variable, we use the relative root mean square error (RMSE) as a measure of accuracy
\begin{align}\label{error-deco}
\varepsilon^{QMC,(k)}_n := \sqrt{\mathbb{E}\left(\bigg|\frac{I_s(\newpart{F}^{(k)})-Q^{\Delta}_{s,n}(\newpart{F}^{(k)})}{I_s(\newpart{F}^{(k)})}\bigg|^2\right)},
\end{align}
where $\mathbb E$ stands for the expectation with respect to the random shifts $\Delta$. The analysis for RMSE, when the integrand is analytic (of Gevrey class with $\delta=1$) can be found \firstcmt{in} \cite{KuoNuyens2016} and \cite{KuoSchwabSloan2012}. In \cite[Lemma 7.4]{ChernovLe2023} we extended this result to integrands that may belong to Gevrey-$\delta$ class with $\delta > 1$. According to that, the RMSE of QMC quadrature for a fixed integer $s$ and $n$ being a power of 2 admits the bound
\begin{equation}\label{errorQMC}
\varepsilon^{QMC,(k)}_n
	\leq C_{s,\vartheta} n^{-\frac{1}{2\vartheta}},
\end{equation}
where $C_{s,\vartheta}$ is independent of $n$ and
\begin{align*}
		\vartheta = 
		\left\{\begin{matrix}
			\omega &\text{for any } \omega \in (\tfrac{1}{2},1) & \text{when } p\in (0,\tfrac{2}{3\delta}],
			\\
			\frac{\delta p}{2-\delta p}    &  & \text{when } p\in (\tfrac{2}{3\delta},\tfrac{1}{\delta}] .
		\end{matrix}\right. 
	\end{align*}


Recall that the summability parameter $p$ can be chosen to satisfy $\frac{1}{5}< p <\frac{2}{3 \delta^{(k)}}$, $k= 1,2$ and therefore $\vartheta$ can be close to~$\frac{1}{2}$ and therefore $\varepsilon_n^{{\rm MC},(k)}$ is close to $n^{-1}$	. This effect is very well visible in the numerical experiments in Figure \ref{fig2}. These results were obtained by solving the variational problem \eqref{variational form} in each quadrature point by the finite element method on a uniform mesh with the mesh size $h=\sqrt{2}/128$ and by means of a fixed-point iteration \eqref{contracting mapping} with the error tolerance of $10^{-14}$ with respect to the $H^1_0(D)$-seminorm. 

The outer expectation in \eqref{errorQMC} is approximated by the empirical mean of $R = 8$ runs, i.e., for $\Delta^{(j)}$, $1 \leq j \leq R$ being an independent sample from the uniform distribution from the unit cube $(0,1)^s$ and $Q^{(j)}_{s,n}(\newpart{F}^{(k)})$ the corresponding QMC quadrature. Thus, we approximate the relative QMC error by 
\begin{equation}
	\varepsilon_n^{{\rm QMC},(k)}\sim
	\sqrt{
		\frac{1}{R} \sum_{j=1}^R
		\brac{\abs{\frac{ I_s^*(\newpart{F}^{(k)})-\newpart{F}^{(j)}_{s,n}(\newpart{F}^{(k)})}{I_s^*(\newpart{F}^{(k)})}}^2}}
		\end{equation}
		and analogously for the standard \newpart{MC} approximation $\varepsilon_n^{{\rm MC},(k)}$.
We choose the reference value $I_s^*(\newpart{F}^{(k)})$ as QMC approximation with a very high number of points, namely $n=2^{15}$, in both cases $k=1,2$. \secondcmt{
It is worth noting that the relative error $\varepsilon_n^{{\rm QMC},(k)}$ is independent of dimension $s$, as shown in, for example, \cite[Lemma 7.4]{ChernovLe2023}.}


Figure \ref{fig2} clearly demonstrates that predicted MC and QMC convergence rates of $n^{-\frac{1}{2}}$ and about $n^{-1}$, cf. \eqref{errorMC} and \eqref{errorQMC}, are very well reproduced in the numerical experiments.

\begin{figure}[h]
	\centerline{\includegraphics[width=0.5\textwidth]{QMC_new_fig.pdf}}
	\caption{Convergence of the quadrature error with respect to the number of samples $n$ for four methods: QMC analytic ($\varepsilon^{{\rm QMC},(1)}_n$), QMC Gevrey ($\varepsilon^{{\rm QMC},(2)}_n$), MC analytic ($\varepsilon^{{\rm MC},(1)}_n$), MC Gevrey ($\varepsilon^{{\rm MC},(2)}_n$).}\label{fig2}
\end{figure}

==> Remedy.tex <==
Observe that the quadratic type nonlinearity $g = f^2$ discussed in the previous section is the simplest, yet very important type of nonlinearity appearing e.g. in Navier-Stokes equations and eigenvalue problems that serve as a model for this paper. The use of Leibniz product rule together with the triangle inequality is a desirable tool that splits the nonlinear part into basic contributions and therefore should be preserved. Instead we seek for an alternative equivalent for \eqref{ana-bound-1d} that can be used in the course of induction. To get a better insight, let's understand whether there is a function $f$ defined in a neighborhood of $J$ of $y_0=0$, such that 
\begin{equation}\label{f2-cond}
	|g^{(n)}(y)| \leq |f^{(n)}(y)| \qquad \forall y \in J, \quad n \in \mN
\end{equation}
is valid for $g = f^2$? The answer is positive and an example of such a function $f$ can be given in closed form
\begin{equation}\label{f2-func}
	f(y) = \tfrac{1}{2}(1-\sqrt{1-y}).
\end{equation}
Indeed, $g(y) = f(y) - \frac{y}{4}$ and hence \eqref{f2-cond} holds as equality for $n \geq 2$. Basic calculations also verify \eqref{f2-cond} for $n = 0$ and $1$. The derivatives of $f$ are all positive for $y<1$ and satisfy
\begin{equation}\label{f2-fallfact}
	2f^{(n)}(y) = (-1)^{n-1}\left(\tfrac{1}{2}\right)\left(\tfrac{1}{2} -1 \right)\dots \left(\tfrac{1}{2}-n + 1\right) (1-y)^{\tfrac{1}{2}-n} = (-1)^{n-1} \left(\tfrac{1}{2}\right)_n (1-y)^{\tfrac{1}{2}-n}
\end{equation}
with the \emph{falling factorial} notation
\begin{equation}\label{def-fallfact}
	(q)_n := \left\{
	\begin{array}{cl}
		1, & n=0, \\
		q(q-1)\dots(q-n+1), & n \geq 1,
	\end{array}
	\right. \qquad q \in \mR.
\end{equation}
For $q<1$ the falling factorial $(q)_n$ is a sing-alternating sequence of $n$. As already indicated in \eqref{f2-func} and \eqref{f2-fallfact}, for our purposes the particular value $q=\frac{1}{2}$ will be important. To further simplify the notation and avoid keeping track of the sign alteration, we denote the \emph{absolute value of the falling factorial of $\frac{1}{2}$} by
\begin{align} 
	\gdnota{n}
	:=
	\left|\left(\tfrac{1}{2} \right)_{n}\right|.
	%	= \frac{1}{2}\frac{1}{2}\frac{3}{2} \dots (n-\frac{3}{2}).
\end{align}
This notation appears somewhat non-standard, but quite convenient, as we will see in the sequel. Notice that the defining property of the Gamma function $\Gamma(z+1) = z\Gamma(z)$ and $\Gamma(\tfrac{1}{2}) = \sqrt{\pi}$ imply the representation
\begin{equation}\label{fallfact-gamma}
	\left[ \tfrac{1}{2} \right]_{n} = \frac{1}{2\sqrt{\pi}}\Gamma(n-\tfrac{1}{2})
	\quad \text{or equivalently} \quad
	n! = \xi_n \gdnota{n} \quad \text{with} \quad \xi_n = 2\sqrt{\pi}\frac{\Gamma(n+1)}{\Gamma(n - \tfrac{1}{2})}
\end{equation}
and the trivial bound
\begin{equation}\label{multiindex-est-2}
	[\tfrac{1}{2}]_{n} \leq n! \leq 2 \cdot 2^n [\tfrac{1}{2}]_{n}.
\end{equation}
Observe next that for $n\geq2$ there holds $g^{(n)}(0) = f^{(n)}(0)$ and therefore this value can be computed in two different ways. On the one hand, it satisfies \eqref{f2-fallfact}, i.e. $g^{(n)}(0) = \tfrac{1}{2}\gdnota{n}$. On the other hand, by the Leibniz product rule
\begin{equation}
	g^{(n)}(0) = \sum_{i=0}^n \binom{n}{i} f^{(i)}(0)f^{(n-i)}(0) = \frac{1}{4}\sum_{i=1}^{n-1} \binom{n}{i} \gdnota{i}\, 
	\gdnota{n-i}.
\end{equation}
Since by definition $\gdnota{0} = 1$, this implies the following combinatorial identities.
\begin{lemma} \label{lem:ff-main-id}
	For all integers $n\geq 2$ the following identities hold
	\begin{equation*}\label{ff-main-id} 
		\sum_{i=1}^{n-1} \binom{n}{i}  
		\gdnota{i}\, 
		\gdnota{n-i}
		=
		2
		\gdnota{n}, \quad
		\sum_{i=1}^{n} \binom{n}{i}  
		\gdnota{i}\, 
		\gdnota{n-i}
		=
		3
		\gdnota{n}, \quad
		\sum_{i=0}^{n} \binom{n}{i}  
		\gdnota{i}\, 
		\gdnota{n-i}
		=
		4
		\gdnota{n}.
	\end{equation*}
\end{lemma}
Remarkably, the constants in the right hand sides of the above identities are uniformly bounded, whereas the constant in the right hand side of \eqref{g2-argument2} grows as $(n+1)$. This suggests to replace the term $n!$ by the falling factorial $[\frac{1}{2}]_n$ in the inductive proof. Moreover, there holds the following alternative characterization of analytic functions.
%\begin{theorem}
%Let $f \in C^\infty(J)$ for some open interval $J$. The function $f$ is in fact real analytic if and only if for every compact set $K \subset I$ there exist constants $C > 0$ and $R > 0$ such that
%\begin{equation}\label{ana-bound-1d}
%|f^{(n)}(y)| \leq \frac{C}{R^n} [\tfrac{1}{2}]_n, \qquad \forall y \in K, \quad n \in \mN_0.
%\end{equation}
%The supremum $r$ of all $R$ satisfying coincides with the radius of convergence of the power series of $f$.
%\end{theorem}
\begin{lemma} \label{lem:ff-main-bound}
	For all integers $n\geq 0$ the following bound hold
	\begin{equation*}\label{ff-main-id} 
		\sum_{i=0}^{n} \binom{n}{i}  
		\gdnota{i}\, 
		\gdnota{n-i}
		\leq
		4
		\gdnota{n}.
	\end{equation*}
\end{lemma}

\begin{theorem}
	Let $f \in C^\infty(I)$ for some open interval $I$. The function $f$ is real analytic if and only if 
	for each $y_0 \in I$, there are an open interval $J$, with
	$y_0 \in J \subseteq I$, and constants $C > 0$ and $R > 0$ such that the derivatives of $f$ satisfy
	\begin{equation}\label{ff-bound-1d}
		|f^{(n)}(y)|\leq \frac{C}{R^n} \gdnota{n}, \qquad \forall y \in J, \quad n \in \mN_0.
	\end{equation}
	The radius of convergence $\rho$ of the power series \eqref{power-series-1d} at some $y_0 \in I$ can be determined as the supremum of $R$ satisfying \eqref{ff-bound-1d}.
\end{theorem} 

\begin{proof} 
	Let us fix $y_0 \in I$. By Theorem \ref{thm:ana-bound-1d} the radius of convergence of the power series \eqref{power-series-1d} at $y_0$ can be written as
	\begin{equation*}
		\rho = \sup\{R~:~ R \text{ satisfies \eqref{ana-bound-1d} with some constant } C = C(R) \}.
	\end{equation*}
	Thus, if we denote
	\begin{equation*}
		\tilde \rho = \sup\{R~:~ R \text{ satisfies \eqref{ff-bound-1d} with some constant } C = C(R) \}
	\end{equation*}
	our aim would be to show that $\rho=\tilde \rho$. On the one hand, there holds $\gdnota{n} \leq n!$. Together with \eqref{ff-bound-1d} this implies \eqref{ana-bound-1d} with the same $R$ and $C$ and thereby $\rho \leq \tilde \rho$. On the other hand, if \eqref{ana-bound-1d} holds, i.e. $f$ is analytic at $y_0 \in I$, the root test shows that the second derivative $f''$ in analytic at $y_0$ too and moreover has the same radius of convergence $\rho$ as the original function $f$, see e.g. \mbox{Proposition 1.1.13} in \cite{Krantz2002}. Now let $n \geq 2$.  By Theorem \ref{thm:ana-bound-1d} this means
	\begin{equation}\label{ddf-ana}
		|f^{(n)}(y)| = |(f''(y))^{(n-2)}(y)| \leq \frac{C}{R^{n-2}} (n-2)!
	\end{equation}
	From definition \eqref{fallfact-gamma} of the falling factorial we find $(n-2)! \leq 4 \gdnota{n}$ and hence \eqref{ddf-ana} implies \eqref{ff-bound-1d} with the same $R$ and $\wtd C := 4 C R^2$
	\begin{equation*}
		|f^{(n)}(y)|\leq \frac{\wtd C}{R^n} \gdnota{n}, \qquad \forall y \in J, \quad n \in \mN_0, \quad n \geq 2.
	\end{equation*} 
	By suitable adjustment of $\wtd C$ the range of $n$ can be extended to cover the cases $n = 0$ and $n = 1$.
	In other words, \eqref{ana-bound-1d} implies \eqref{ff-bound-1d} with the same $R$ and possibly adjusted $C$. This imples $\rho \geq \tilde \rho$ and thereby finishes the proof. 
	%\begin{equation}
	%|f^{(n)}(y)| \leq \frac{C}{R^n} \xi_n [\tfrac{1}{2}]_n \leq \frac{2C}{(R/2)^n} \gdnota{n}
	%\end{equation}
	%since $\xi_n \leq 2^{n+1}$. Thus, \eqref{ff-bound-1d} follows with $C$ and $R$ replaced by $2C$ and $R/2$.
\end{proof}

==> abstract.tex <==
	We investigate a class of parametric elliptic eigenvalue problems with homogeneous essential boundary conditions where the coefficients (and hence the solution $u$) may depend on a parameter $\vy$. For the efficient approximate evaluation of parameter sensitivities of the first eigenpairs on the entire parameter space we propose and analyze Gevrey class or analytic regularity of the solution with respect to the parameters. This result has immediate implications for convergence of various numerical schemes for  parametric elliptic eigenvalue problems, in particular, for elliptic eigenvalue problems with infinitely many parameters arising from elliptic differential operators with random coefficients.

==> higher_regularity.tex <==
\tl{
In connection with numerical approximations of the problem \eqref{gen equation} in the domain $D$, it is of interest to establish sufficient conditions on the data which imply additional regularity of the parametric solutions in $D$, while maintaining the summability of their series expansions. From now, we assume \ac{additionally} that
\begin{align*}
f\in L^2(D)
\quad
\text{ and }
a\in W^{1,\infty}(D)
\end{align*} 
\begin{lemma}
\label{general upper bound for um derivative}
	For any fixed $\vmu\in \cF$, $m^*=2m$ \todo{do we need $2m$ here?} and $(d,m^*-1)\in \cM$, suppose that \eqref{u V norm ref} holds for all multi index  $\vell\leq \vmu$, i.e.
	\begin{align}\label{uV assumption}
		\norm{\partial^{\vell} u (\vy)}{V}
		\leq
		\frac{C_u \rho^{\abs{\vell}} \gdnota{\abs{\vell}}}{\vR^{{\vell}}} (\abs{\vell}!)^{\delta-1} \qall \vell \leq \vmu.
	\end{align}
For all positive \ac{integers} $k\leq m^*$  we define 
\begin{align}
\cL^*_{k}:= 
 L^{\frac{m^*}{k}}(D) 
\end{align}
Then, the following estimates are valid
	\begin{equation} \label{um derivative Lk}
		\norm{\partial^{\vmu}(u(\vy)^k)}{\cL^*_k}
		\leq
		\frac{4^{k-1}(C_{m^*}\,C_m^{-1}\,C_u)^{k}\, \rho^{\abs{\vmu}} \gdnota{\abs{\vmu}}}{\vR^{{\vmu}}}
		(\abs{\vmu}!)^{\delta-1}.
	\end{equation}
\end{lemma}
\begin{proof}
For base of induction, we check $k=1$, indeed we have
\begin{align*}
\norm{\partial^{\vmu}(u(\vy))}{\cL^*_1}
=
\norm{\partial^{\vmu}(u(\vy))}{L^{m^*}(D)}
\leq
C_{m^*}\,C_m^{-1} \norm{\partial^{\vmu}(u(\vy))}{V}
\leq
	\frac{C_{m^*}\,C_m^{-1}\,C_u\, \rho^{\abs{\vmu}} \gdnota{\abs{\vmu}}}{\vR^{{\vmu}}} (\abs{\vmu}!)^{\delta-1}.
\end{align*}
 For the inductive step, we now assume that \eqref{um derivative Lk} holds for all number $k\leq n$ such that $n\leq \ac{m^*}-1$, and prove that this implies the same bound for $k = n+1$. Applying Leibniz general product rule to $u^{n+1} = u^n\,u$ and the triangle inequality, we arrive at
\begin{align*}
	\norm{\partial^{\vmu}(u^{n+1})}{\cL^*_{n+1}}
	=
	\norm{
	\sum_{\vzero \leq \vell\leq \vmu}
		\brac{\vmu \atop \vell}
		\partial^{\vell}(u^{n})
	\partial^{\vmu-\vell}u
	}{\cL^*_{n+1}}
\leq
	\sum_{\vzero \leq \vell\leq \vmu}
\brac{\vmu \atop \vell}
	\norm{
	\partial^{\vell}(u^{n})
	\partial^{\vmu-\vell}u
}{\cL^*_{n+1}}.
\end{align*} 
By the H\"older inequality \eqref{adjusted Hoelder} with $w=\partial^{\vell}(u^{n})$, $v=\partial^{\vmu-\vell}u$, $p=n$, $q=1$ and recalling the inductive assumption for the individual terms we obtain
\begin{align*}
	\norm{\partial^{\vmu}(u^{n+1})}{\cL^*_{n+1}}
	&\leq
	\sum_{\vzero \leq \vell\leq \vmu}
	\brac{\vmu \atop \vell}
	\norm{
		\partial^{\vell}(u^{n})
	}{\cL^*_{n}}
\norm{
	\partial^{\vmu-\vell}u
}{\cL^*_{1}}\\
&\leq
	\sum_{\vzero \leq \vell\leq \vmu}
\brac{\vmu \atop \vell}
\brac{	\frac{4^{n-1}(C_{m^*}\,C_m^{-1}\,C_u)^{n}\, \rho^{\abs{\vell}} \gdnota{\abs{\vell}}}{\vR^{{\vell}}}(\abs{\vell}!)^{\delta-1}}
\brac{\frac{C_{m^*}\,C_m^{-1}\,C_u\, \rho^{\abs{\vmu-\vell}} \gdnota{\abs{\vmu-\vell}}}{\vR^{{\vmu-\vell}}}(\abs{\vmu-\vell}!)^{\delta-1} }\\
&=
\frac{4^{n-1}(C_{m^*}\,C_m^{-1}\,C_u)^{n+1} \rho^{\abs{\vmu}}}{\vR^{{\vmu}}}
\sum_{\vzero \leq \vell\leq \vmu}
\brac{\vmu \atop \vell}
\gdnota{\abs{\vell}}
\gdnota{\abs{\vmu-\vell}}
\abs{\vell}!^{\delta-1}
\abs{\vmu-\vell}!^{\delta-1}\\
&\leq
\frac{4^{n}(C_{m^*}\,C_m^{-1}\,C_u)^{n+1} \rho^{\abs{\vmu}}}{\vR^{{\vmu}}}
\gdnota{\abs{\vmu}}
\abs{\vmu}!^{\delta-1},
\end{align*}
where we have used \eqref{multiindex-est-1} and \eqref{multiindex-est-3} in the last step. This finishes the proof.
\end{proof}
\begin{lemma}
\label{upper bound for um derivative L2}
	For any fixed $\vmu\in \cF$ and $(d,2m-1)\in \cM$, suppose that \eqref{u V norm ref} holds for all multi index  $\vell\leq \vmu$, i.e.
	\begin{align}\label{uV deri L2}
		\norm{\partial^{\vell} u (\vy)}{V}
		\leq
		\frac{C_u \rho^{\abs{\vell}} \gdnota{\abs{\vell}}}{\vR^{{\vell}}} (\abs{\vell}!)^{\delta-1} \qall \vell \leq \vmu.
	\end{align}
Then, for all natural \ac{numbers $m$ satisfying} \eqref{cond: m d restriction} the following estimates are valid
	\begin{equation} \label{um derivative L2}
		\norm{\partial^{\vmu}(u(\vy)^m)}{L^2(D)}
		\leq
		\frac{4^{m-1}(C_{m^*}\,C_m^{-1}\,C_u)^{m}\, \rho^{\abs{\vmu}} \gdnota{\abs{\vmu}}}{\vR^{{\vmu}}}
		(\abs{\vmu}!)^{\delta-1}.
	\end{equation}
\end{lemma}
\begin{proof}
Notice that $L^2(D)=\cL^*_{m}$ and employ Lemma \ref{general upper bound for um derivative} we have
\begin{align*}
	\norm{\partial^{\vmu}(u^{\ac{m}})}{L^{2}(D)}
	=
	\norm{
	\partial^{\vmu}(u^{m})
}{\cL^*_{m}}
\leq
\frac{4^{m-1}(C_{m^*}\,C_m^{-1}\,C_u)^{m}\, \rho^{\abs{\vmu}} \gdnota{\abs{\vmu}}}{\vR^{{\vmu}}}
		(\abs{\vmu}!)^{\delta-1}.
\end{align*}
we finish the proof.
\end{proof}
}

==> higher_spatial_regularity.tex <==
\subsection{Parametric regularity in $H^2(D)$ and pointwise estimates}

If $D$ is a convex Lipschitz domain and the coefficients $a,b$ and the right-hand side $f$ are sufficiently regular, it is actually possible to prove that estimates of the type \eqref{u H1 norm ref} remain valid in $H^2(D)$, and therefore in every space containing $H^2(D)$ with continuous embedding. In particular, pointwise estimates follow from $L^\infty(D)$ bounds. 

If the data are sufficiently regular (see Assumption \ref{Assumption1} below for the precise regularity assumptions), we recall the cariational formulation \eqref{variational form} and take $\vnu$-th derivative its both sides with respect to $\vy$
\begin{equation*}
 {C_m^2} \int_D \partial^{\vnu} (a \nabla u)\cdot \nabla v = \int_D \partial^{\vnu}(  {C_m} \,f - b u^m ) v.
\end{equation*}
The Leibniz product rule and formal  
integration by parts delivers
\begin{equation*}
 {C_m^2}\int_D a (\Delta \partial^{\vnu} u) v = \int_D \left(\partial^{\vnu}\big(b u^m \big) - {C_m^2} \nabla a \cdot \nabla  \partial^{\vnu} u - C_m \partial^{\vnu} f \right) v 
  +
 {C_m^2}\sum_{\vzero \leq \veta < \vnu }
\binom{\vnu}{\veta} \partial^{\vnu-\veta} a\, \nabla \partial^{\veta} u \cdot \nabla v.
\end{equation*}

We now let $v = \Delta \partial^{\vnu} u$ and apply the triangle and the Cauchy-Schwarz inequalities. Recall that $a\geq 1$, and hence
\begin{equation}\label{vnu-Delta-u}
\|\Delta \partial^{\vnu} u\|_{L^2(D)}
\leq \| C_m^{-2} \partial^{\vnu} \big( b u^m\big) - \nabla a \cdot \nabla \partial^{\vnu}  u -  {C_m^{-1}\,} \partial^{\vnu}  f\|_{L^2(D)} 
+ \sum_{\vzero \leq \veta < \vnu }
\binom{\vnu}{\veta} \|\partial^{\vnu-\veta} a\|_{L^\infty(D)} \|\nabla \partial^{\veta} u\|_{L^2(D)}.
\end{equation}

The second term admits Gevrey-$\delta$ bounds if $L^\infty(D)$ and $V^*$-norms for $a$ and $f$ in Assumption \ref{Assumption} are replaced by the $W^{1,\infty}(D)$ and $L^2(D)$-norms respectively. More precisely, we replace Assumption \ref{Assumption} by the following.
	\begin{assumption} \label{Assumption1}
		For all fixed values $\vy\in U \in \mR^s$ with $s<\infty$, the coefficients $a(\vy) \in W^{1,\infty}(D)$, $b(\vy) \in L^\infty(D)$ and $f(y)\in L^2(D)$. Moreover, for all $\vnu\in \mN^s$ there exist positive constants $\vR=(R_1,R_2,\dots)$ independent of $s$ such that
		\begin{align*}
			\norm{\partial^{\vnu} a(\vy)}{W^{1,\infty}(D)}
			\leq
			\frac{\overline{a}}{2}
			\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}} , \qquad
			\norm{\partial^{\vnu} b(\vy)}{L^\infty(D)}
			\leq
			\frac{\overline{b}}{2}
			\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}} , \qquad
			\norm{\partial^{\vnu} f(\vy)}{L^2(D)}
			\leq
			\frac{\overline{f}}{2}
			\frac{(\abs{\vnu}!)^\delta }{(2\vR)^{\vnu}}  .
		\end{align*} 
Assume moreover, that $m \in \mN$ is such that $H^1(D)$ is continuously embedded into $L^{2m}(D)$, i.e. $(d,2m-1) \in \cM$, see \eqref{cond: m d restriction}.
	\end{assumption}
According to \eqref{ff-estimates} Assumption \ref{Assumption1} implies
\begin{align}\label{abf1 assumption}
	\norm{\partial^{\vnu} a(\vy)}{W^{1,\infty}(D)}
	\leq
	\frac{\overline{a} \gdnota{\abs{\vnu}}}{\vR^{\vnu}} (\abs{\vnu}!)^{\delta-1} , \qquad
	\norm{\partial^{\vnu} b(\vy)}{L^\infty(D)}
	\leq
	\frac{\overline{b} \gdnota{\abs{\vnu}}}{\vR^{\vnu}}
	(\abs{\vnu}!)^{\delta-1} , \qquad
	\norm{\partial^{\vnu} f(\vy)}{L^2(D)}
	\leq
	\frac{\overline{f} \gdnota{\abs{\vnu}}}{\vR^{\vnu}}(\abs{\vnu}!)^{\delta-1}.
\end{align}
 The regularity of $\Delta \partial^{\vnu} u$ can now be established by bounding the terms in the right-hand side of \eqref{vnu-Delta-u}. The Leibniz general product rule and the triangle inequality yield for the first term 
\begin{equation*}
\begin{split}
\|\partial^{\vnu} ( {C_m^{-2}} b u^m - \nabla a \cdot \nabla u -  {C_m^{-1}}\,f)\|_{L^2(D)}
&\leq 
 {C_m^{-1}} \|\partial^{\vnu} f\|_{L^2(D)}
+
\sum_{\vzero \leq \veta \leq \vnu} \binom{\vnu}{\veta}
\big(
 {C_m^{-2}}\|\partial^{\vnu-\veta} b\|_{L^\infty(D)} \|\partial^{\veta} (u^m)\|_{L^2(D)}
+ \|\nabla \partial^{\vnu-\veta} a\|_{L^\infty(D)} \|\nabla \partial^{\veta} u\|_{L^2(D)}
\big)\\
&\leq 
 {C_m^{-1}}\|\partial^{\vnu} f\|_{L^2(D)}
+
\frac{(|\vnu|!)^{\delta-1}}{\vR^{\vnu}}
\sum_{\vzero \leq \veta \leq \vnu} \binom{\vnu}{\veta}
\big(
4^{m-1}(C_{2m-1} C_m^{-1}  C_u)^m  {C_m^{-2}} \overline{b} +  C_m^{-1} C_u \overline{a}
\big) \rho^{|\veta|} \gdnota{|\vnu-\veta|} \gdnota{|\veta|}\\
&\leq 
 {\big(
4^{m}(C_{2m-1} C_u)^m C_m^{-m-2}  \overline{b}  + 4C_m^{-1} C_u \overline{a} + C_m^{-1} \overline{f}
\big)}
\frac{  \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1},
\end{split}
\end{equation*}
In the above estimate we used \eqref{multiindex-est-3} and the bounds
\begin{equation*}
\|\partial^{\veta} u\|_{L^{2m}(D)} 
\leq C_{2m-1}
\|\partial^{\veta} u\|_{H^1_0(D)} 
= C_{2m-1} C_m^{-1}
\|\partial^{\veta} u\|_V
\leq C_{2m-1} C_m^{-1}  C_u 
\frac{ \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1},
\end{equation*}
i.e. the Sobolev embedding for $(d,2m-1) \in \cM$ and Theorem \ref{gevrey regularity for semilinear}. By Lemma \ref{upper bound for f derivative} this implies
\begin{equation*}
\|\partial^{\veta} (u^m)\|_{L^2(D)} 
=
\|\partial^{\veta} (u^m)\|_{\LL{2m}{m}} 
\leq 
4^{m-1} (C_{2m-1} C_m^{-1}  C_u)^m
\frac{ \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1}.
\end{equation*}
The argument can now be completed by an inductive argument, which is the subject of the following Theorem.

\begin{theorem}\label{thm:2}
Suppose the assumptions of Theorem \ref{gevrey regularity for semilinear} hold and additionally Assumption \ref{Assumption1} is satisfied. Then $\Delta \partial^{\vnu} u \in L^2(D)$  for all $\vnu \in \cF$ and there holds
\begin{equation}\label{Delta-u-derivative}
\|\Delta \partial^{\vnu}u\|_{L^2(D)} \leq 
\frac{2C_{\Delta} \tilde{\rho}^{|\vnu|} \gdnota{|\vnu|}}{\vR	^{\vnu}} (|\vnu|!)^{\delta-1},
\end{equation}
where $C_\Delta :=   {
4^{m}(C_{2m-1} C_u)^m C_m^{-m-2}  \overline{b}  + 4C_m^{-1} C_u \overline{a} + C_m^{-1} \overline{f}
}$ and $\tilde \rho := \max(6\overline{a},\rho)$.
\end{theorem}

\begin{proof}
We prove the statement by induction. For $\vnu = \vzero$ we have by \eqref{vnu-Delta-u}
\begin{equation*}
\begin{split}
\|\Delta u\|_{L^2(D)} &\leq \| {C_m^{-2}} bu^m - \nabla a \cdot \nabla u -  {C_m^{-1}} f\|_{L^2(D)}
\leq  {C_m^{-2}} \|b\|_{L^\infty(D)} \|u^m\|_{L^2(D)} 
+ \|\nabla a\|_{L^2(D)} \|\nabla u\|_{L^2(D)}
+  {C_m^{-1}} \|f\|_{L^2(D)}\\
&\leq 
 {C_m^{-2}}\overline{b} \|u\|^m_{L^{2m}(D)}
+\overline{a} \|\nabla u\|_{L^2(D)} + {C_m^{-1}} \overline{f}
\leq  {C_m^{-2}} \overline{b} (C_{2m-1}  C_m^{-1}\|u\|_V)^m
+\overline{a}  C_m^{-1} \|u\|_V +  {C_m^{-1}} \overline{f} \\
&\leq 
 {C_m^{-2}}(C_{2m-1} C_m^{-1} C_u)^m \overline{b} 
+ C_m^{-1}C_u \overline{a}  +  {C_m^{-1}}\overline{f} \leq  {2 C_\Delta}
\end{split}
\end{equation*}

The aim is now to prove \eqref{Delta-u-derivative}, assuming that it is valid for all derivatives of order strictly less than $\vnu$. From \eqref{vnu-Delta-u} and the bound below it, we readily have for $|\vnu|\geq 1$
\begin{equation*}
\begin{split}
\|\Delta \partial^{\vnu} u\|_{L^2(D)}
&\leq 
C_\Delta
\frac{  \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1} +
\sum_{\vzero \leq \veta < \vnu }
\binom{\vnu}{\veta} \|\partial^{\vnu-\veta} a\|_{L^\infty(D)} \|\Delta \partial^{\veta} u\|_{L^2(D)}\\
&\leq 
C_\Delta
\frac{  \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1} +
\sum_{\vzero \leq \veta < \vnu }
\binom{\vnu}{\veta} 
\frac{\overline{a}\gdnota{|\vnu-\veta|}}{\vR^{\vnu-\veta}} (|\vnu-\veta|!)^{\delta-1} 
\frac{2C_\Delta \tilde{\rho}^{|\veta|}\gdnota{|\veta|}}{\vR^{\veta}} (|\veta|!)^{\delta-1} \\
&\leq 
2C_\Delta
\frac{  \rho^{|\vnu|} \gdnota{|\vnu|} }{\vR^{\vnu}}(|\vnu|!)^{\delta-1} \big(\frac{1}{2} + \frac{3\overline{a}}{\tilde \rho}\big).
\end{split}
\end{equation*}
According to the definition of $\tilde \rho$ the term in the  parentheses is bounded by 1 and the claim of the theorem follows.
\end{proof}

Finally we remark that $(\|u\|_{L^2(D)}^2 + \|\Delta u\|_{L^2(D)}^2)^{1/2}$ is an equivalent norm on $H^2(D) \cap H^1_0(D)$. Moreover, if $D$ is convex, the solution $u \in H^1_0(D)$ to \eqref{variational form} is in $H^2(D)$ by the  linear elliptic regularity theory, see e.g. \cite{Grisvard1985}. Indeed, the solution $u\in H^1_0(D)$ to \eqref{variational form} can be seen as the unique solution of
\[
\int_D a \nabla w \cdot \nabla v = \int_D \tilde f v, \qquad \forall v \in H^1_0(D),
\]
where $\tilde f := f - b u^m$. Since $H^1_0(D)$ is continuously embedded in $L^{2m}(D)$ and $\tilde f \in L^2(D)$, the linear elliptic regularity theory in convex domains applies. As a result we have in this case
\[
\|u\|_{H^2(D)} \lesssim (\|u\|_{L^2(D)}^2 + \|\Delta u\|_{L^2(D)}^2)^{1/2} \leq ((C_m^{-1}C_u)^2  +  (2C_\Delta)^2)^{1/2} \frac{ (|\vnu|!)^{\delta}}{(\vR/\tilde \rho)^{\vnu}}.
\]


==> multi_index.tex <==
The following  standard \secondcmt{multi-index} notations will be used in what follows, see e.g. \cite{BoutetDeMonvel1967,CohenDevoreSchwab2010}. We denote the countable set of finitely supported sequences of nonnegative integers by
\begin{equation}\label{cF-def}
	\cF := 
	\left\{
	\vnu =(\nu_1,\nu_2,\dots)~:~ \nu_j\in \mN_0,
	\text{ and } \nu_j \neq 0
	\text{ for only a finite number of } j
	\right\}  \subset \mN^{\mN},
\end{equation}
where the summation $\valpha + \vbeta$ and the partial order relations $\valpha < \vbeta$ and $\valpha \leq \vbeta$ of elements in $\valpha, \vbeta \in \cF$ are understood componentwise. We write
\begin{align*}
	\abs{\vnu}
	:=
	\sum_{j\geq 1} \nu_j, 
	\qquad \qquad
	\vnu!
	:=
	\prod_{j\geq 1} v_j!, 
	\qquad \qquad
	\vR^{\vnu}= \prod_{j\geq 1} R_j^{v_j}
\end{align*}
for the absolute value, the multifactorial and the power with the \secondcmt{multi-index} $\vnu$ and a sequence $\vR=\{R_j\}_{j\geq 1}$ of positive real numbers. Notice that $\abs{\vnu}$ is finite if and only if $\vnu\in \cF$. For $\vnu\in \cF$ supported in $\sett{1,2,\dots, n}$, we define the partial derivative with respect to the variables $\vy$
\begin{align*}
	\partial^{\vnu} u
	=
	\frac{\partial^{\abs{\vnu}}u}
	{\partial y_1^{\nu_1} \partial y_2^{\nu_2} \dots \partial y_n^{\nu_n}}.
\end{align*}
For two \secondcmt{multi-indicies} $\vnu, \veta \in \cF$ we define the binomial coefficient by
\begin{equation*}
\brac{\vnu \atop \veta}  = 
	\prod_{j\geq 1}  \brac{\nu_j \atop \eta_j}.
\end{equation*}

The above \secondcmt{multi-index} notations are handy for treatment of multiparametric objects. The following technical Lemma is instrumental for the forthcoming analysis.
\begin{lemma}
	For two \secondcmt{multi-indicies} $\vnu, \veta\in \cF$ satisfying $\veta \leq \vnu$, a unit \secondcmt{multi-index} $\ve$ and $\delta \geq 1$ we have
	\begin{equation}\label{multiindex-est-1}
		(|\vnu-\veta|!)^{\delta-1} (|\veta|!)^{\delta-1} \leq (|\vnu|!)^{\delta-1},
	\end{equation}
	\begin{equation}
		\sum_{\newpart{0<\veta < \vnu}}
		\brac{\vnu \atop \veta} 
		\gdnota{|\veta|}
		\gdnota{|\vnu-\veta|}
		\leq
		\newpart{2} [\tfrac{1}{2}]_{|\vnu|},\label{multiindex-est-7}
	\end{equation}
	\begin{equation}
		\newpart{\sum_{0<\veta \leq \vnu}
		\brac{\vnu \atop \veta} 
		\gdnota{|\veta|}
		\gdnota{|\vnu-\veta|}
		\leq
		3 [\tfrac{1}{2}]_{|\vnu|}},\label{multiindex-est-3}
	\end{equation}
	\begin{equation}
	\sum_{\newpart{\vzero< \veta \leq \vnu}}
	\brac{\vnu\atop\veta}
	\gdnota{\abs{\vnu+\ve-\veta}}
	\gdnota{\abs{\veta}}
	\leq\newpart{
	\gdnota{\abs{\vnu+\ve}}},
	\label{multiindex-est-6}
\end{equation}
\begin{equation}
	\sum_{\vzero< \veta \leq \vnu}
	\sum_{\newpart{\vzero< \vell \leq \veta}}
	\brac{\vnu\atop\veta}
	\brac{\veta\atop \vell}
	\gdnota{\abs{\veta-\vell}}
	\gdnota{\abs{\vell}}
	\gdnota{\abs{\vnu+\ve-\veta}}
	\leq
	\newpart{3}\gdnota{\abs{\vnu+\ve}}.
	\label{multiindex-est-5}
\end{equation}
\end{lemma}
\begin{proof}
	Notice that for two non-negative integers $n!\cdot m! \leq (n+m)!$ and therefore % implying for $\delta \geq 1$
	\begin{align*}
|\vnu-\veta|! |\veta|!
		\leq
(|\vnu-\veta|+ |\veta|)!
		= 		|\vnu|!.
	\end{align*}
	Since $(\cdot)^{\delta -1}$ is an increasing function for $\delta \geq 1$, the estimate \eqref{multiindex-est-1} follows.
	According to \cite[Lemma 7.1]{ChernovLe2023}, we have
	\begin{align}\label{iden: Chu-Vandermonde}
	\sum_{\abs{\veta}=r \atop \eta \leq \vnu} \brac{\vnu \atop \eta}= \brac{|\vnu| \atop r},
	\end{align}
which is sometimes called generalized Vandermonde or Chu-Vandermonde identity.
This together with \eqref{ff-bound-3} imply the estimate
\begin{align*}
	\sum_{\newpart{0<\veta < \vnu}}
	\brac{\vnu \atop \veta} 
	\gdnota{|\vnu-\veta|}
	\gdnota{|\veta|}
	=
	\sum_{\newpart{r=1}}^{\newpart{\abs{\vnu}-1}}
	\sum_{\abs{\veta}=r \atop \veta \leq \vnu} \brac{\vnu \atop \veta}
	\gdnota{|\vnu|-r}
	\gdnota{r}
	=
	\sum_{\newpart{r=1}}^{\newpart{\abs{\vnu}-1}}
	\brac{|\vnu| \atop r} 
	\gdnota{|\vnu|-r}
	\gdnota{r}
	\leq
	\newpart{2}\gdnota{|\vnu|}.
\end{align*}
It shows inequality \eqref{multiindex-est-3}. Similarly, we derive bounds \eqref{multiindex-est-3} and \eqref{multiindex-est-6} by applying \eqref{iden: Chu-Vandermonde} to \eqref{ff-bound-3} and \eqref{ff-bound-1}, respectively. The final estimate \eqref{multiindex-est-5} follows by consecutive application of \eqref{multiindex-est-3} and  \eqref{multiindex-est-6}.
\end{proof}


==> new_intro.tex <==
Elliptic semilinear problems arise in numerous applications in natural sciences and engineering. Prominent examples are reaction-diffusion-type problems with nonlinear reaction (reproduction) terms for modelling of various processes such as phase separation, combustion, soil-moisture-physics, biological population genetics, etc. For analysis of parametric semilinear problems we refer to works by Hansen and Schwab \cite{HansenSchwab13}, where the particular case of a stochastic parameter perturbation has been addressed, see also the recent work \cite{bahn2023semilinear} for semilinear eigenvalue problems under uncertainty. The regularity of the solution of the problem with respect to the parameter is important for construction of efficient numerical approximations in the parameter domain. For example, if the quantity of interest is solution's average value over a prescribed parameter domain, Monte Carlo and Quasi-Monte Carlo methods can be applied for the numerical integration. However, the use of Quasi-Monte Carlo integration does only pay off if the solution features certain higher regularity properties. \secondcmt{In this paper, we investigate the parametric regularity of the solution's  for a semilinear problem, focusing on two norms: $H^1_0(D)$ and $H^2(D)$.  Subsequently, we illustrate their implications in Gauss-Legendre quadrature and random shift lattice rules through numerical experiments.}



Let us consider a prototypic real second-order elliptic semilinear partial differential equation of the general form
\begin{equation}\label{gen equation}
	\begin{split}
		-C_m^2\nabla\cdot (\va(\vx,\vy)\nabla u(\vx,\vy))
		+b(\vx,\vy) \left[u(\vx,\vy)\right]^m
		&=
		C_m\,f(\vx,\vy) \hspace*{24mm}  (\vx,\vy)\in D \times U, 	\\
		u(\vx,\vy)&=0 \hspace*{35mm} 
		(\vx,\vy) \in \partial D \times U, %\notag
	\end{split}
\end{equation}
where the derivative operator $\nabla$ acts in the physical variable $\vx \in D$, where $D$ is a bounded Lipschitz domain in $\mR^d$. The above semilinear problem could be reduced to linear by choosing $b\equiv 0$ or $m= 1$. \newpart{For the parametric regularity of linear problems, refer to works such as  \cite{CohenDevoreSchwab2010,CohenDevoreSchwab2011,KuoSchwabSloan2012}}. The vector of parameters $\vy = (y_1,y_2,\dots) \in U$ has either finitely many or countably many components. For example, if $\vy$ is a random parameter, the model with $U:= [-\frac{1}{2},\frac{1}{2}]^{\mN}$ and $\vy \in U$ being a countably-dimensional vector of independently and identically distributed uniform random variables has been frequently used in the literature \cite{CohenDevoreSchwab2010,CohenDevoreSchwab2011,KuoSchwabSloan2013,KuoNuyens2016}.
%The necessary restrictions on the power $m\in \mN$ and the dimension $d$ of the domain $D$ are in the range \eqref{cond: m d restriction} throughout this paper and denote the corresponding set of parameters $(d,m)$ by $\cM$ as following, cf. \cite{HansenSchwab13}
The necessary restrictions on the power $m\in \mathbb{N}$ and the dimension $d$ of the domain $D$ fall within the range specified in \eqref{cond: m d restriction} throughout this paper. We denote the corresponding set of parameters $(d,m)$ by $\mathcal{M}$, as outlined in \cite{HansenSchwab13}
\begin{equation}\label{cond: m d restriction}
\begin{split}
	d=1 \text{ or } d=2:& \quad m\in \mN \\
	d=3: H^1_0(D) \hookrightarrow L^6(D)& \quad \text{hence } 1\leq m\leq 5\\
	d=4: H^1_0(D) \hookrightarrow L^4(D)& \quad \text{hence } 1\leq m\leq 3\\
	d=5: H^1_0(D) \hookrightarrow L^{10/3}(D)& \quad \text{hence } 1\leq m\leq 2\\
	d=6: H^1_0(D) \hookrightarrow L^3(D)& \quad \text{hence } 1\leq m\leq 2\\
	 d\geq 7:& \quad m=1,
\end{split}
\end{equation}
and $C_m$ is the constant of Sobolev embedding $H^1_0(D)\hookrightarrow L^{m+1}(D)$, see e.g. \cite{Mizuguchi2017}. Clearly, the rescaling of \eqref{gen equation} with $C_m$ is made for the sake of convenience and has no effect in the parametric regularity of the solution. Without loss of generality, in the following we assume that the coefficients $a(\cdot,\vy),b(\cdot,\vy)$ and $\norm{f(\cdot,\vy)}{H^{-1}(D)}$ admit the uniform bounds
\begin{equation}\label{ab-bounds}
		1 \leq a(\vx,\vy)\leq\frac{\overline{a}}{2} , \qquad
		 \abs{b(\vx,\vy)} \leq \frac{\overline{b}}{2}, \qquad
		 \norm{f(\cdot,\vy)}{H^{-1}(D)} \leq \frac{\overline{f}}{2}	 
\end{equation}
for all $\vy \in U$ and almost all $\vx \in D$. Thus, for every fixed $\vy \in U$ and under a reasonable assumption, the problem \eqref{gen equation} is well-posed, see for example \cite{HansenSchwab13}. Since the coefficients depend on the parameters $\vy$, the solution $u$ will depend on $\vy$ as well. Particularly, if $\vy$ is random, then $u(\vx,\vy)$ will be random too.


In this paper we present a rigorous regularity analysis for the solution $u$ with respect to the parameter $\vy$ in the general case where the given data $a, b$ and $f$ are infinitely differentiable functions of $\vy$ belonging to the Gevrey class $G^{\delta}$ for some fixed $\delta \geq 1$. The scale of Gevrey classes is a nested scale of the parameter $\delta$ that fills the gap between analytic and $C^\infty$  functions 
\begin{equation} \label{Gdelta-nested}
\secondcmt{\cA= G^{1} \subset}\, G^{\delta} \subset G^{\delta'} \subset C^\infty, \qquad \secondcmt{1 < \delta < \delta'}. 
\end{equation}
The case of analytic functions (i.e. \secondcmt{$\cA=G^{1}$,} Gevrey-$\delta$-class function with $\delta = 1$) is the simplest and arguably most important of this scale and has been addressed for parametric/stochastic semilinear problem before, see \cite{HansenSchwab13}. The above mentioned work considers the coefficient of the type of the affine parametrization and prove the analyticity of the solution using elegant complex analysis arguments.

Besides the complex variable argument, the real-variable argument is also has been used as a powerful tool to achieve analytic regularity. For the analysis of the eigenvalue problems we refer to \cite{Gilbert2019}. However, the direct application of the real-variable argument typically leads to suboptimal estimates. To overcome this, in \cite{ChernovLe2023}, we suggest a modified argument, namely \emph{alternative-to-factorial technique}, and obtain optimal regularity for the eigenvalue problem. The aim of this paper is to introduce this approach and enhance it in the case of the parametric semilinear problems. 

The structure of the paper is as follows. In Section \ref{sec: Remedy} we introduce the falling factor notation, which is the main tool for our \emph{alternative-to-factorial technique} first introduced in \cite{ChernovLe2023}. In Section \ref{sec: Gevrey} we introduce Gevrey-class function and formulate the regularity assumptions on the coefficients of the semilinear problem \eqref{gen equation}. In Section \ref{sec:EVPtheory} we summarize the properties of elliptic semilinear problems needed for the forthcoming regularity analysis. In Section~\ref{sec: main result} we present the proof of the main results, namely the Gevrey-$\delta$ class regularity for the solution with respect to the $H^1_0(D)$-seminorm in Theorem \ref{gevrey regularity for semilinear} and the higher spatial regularity results in Theorem \ref{thm:2}. The meaning and validity of the main regularity results is illustrated by the applications and numerical experiments in Section~\ref{sec: num exp}. 

